Which Dwarf Is This? Doppeldwarf-306 and Near-Identical Instance Retrieval

Most established instance-retrieval benchmarks emphasise landmarks; small sculptures from visually similar series offer a complementary challenge. We introduce Doppeldwarf-306: 1,691 openly licensed photographs of 306 bronze dwarf statues in Wroc{\l}aw, Poland, many made in themed series that share one style, with the photographer of each image recorded. With no training, nearest-neighbour search over frozen DINOv2 features names the right statue first for 93.1% of leave-one-out queries, and the best of thirteen backbones from seven pretraining paradigms reaches 94.7%. Accuracy falls slowly as candidates are added: for DINOv2, by about 0.8 points each time their number doubles. A natural design for a phone guide compares a photograph only with statues near the user. In simulation this helps, but less than an equal number of randomly chosen statues does, so random subsampling overstates its value; a permutation test ties the penalty to the real layout (p = 0.005). Used as a weight instead of a filter, location raises DINOv2 from 93.4% to 98.7% for a simulated user 25 m from the statue. With the query's photographer withheld, learned local-feature matching raises DINOv2 accuracy from 81.8% to 85.5% and also improves DINOv3. Comparing the two best candidates cuts DINOv2's false acceptance of unknown statues from 38.3% to 19.6% at 90% known acceptance.

==> generated/extra-numbers.tex <==
\makeatletter
\@namedef{wv@cg3_camera_median_references@v}{600.0}
\@namedef{wv@cg3_camera_queries@v}{1565}
\@namedef{wv@cg3_camera_top_1@v}{94.8}
\@namedef{wv@cg3_camera_top_1@ci}{93.5 to 95.8}
\@namedef{wv@cg3_camera_top_1@lo}{93.5}
\@namedef{wv@cg3_camera_top_1@hi}{95.8}
\@namedef{wv@cg3_camera_top_5@v}{97.2}
\@namedef{wv@cg3_camera_top_5@ci}{96.2 to 97.9}
\@namedef{wv@cg3_camera_top_5@lo}{96.2}
\@namedef{wv@cg3_camera_top_5@hi}{97.9}
\@namedef{wv@cg3_phone_median_references@v}{700.0}
\@namedef{wv@cg3_phone_queries@v}{51}
\@namedef{wv@cg3_phone_top_1@v}{90.2}
\@namedef{wv@cg3_phone_top_1@ci}{79.0 to 95.7}
\@namedef{wv@cg3_phone_top_1@lo}{79.0}
\@namedef{wv@cg3_phone_top_1@hi}{95.7}
\@namedef{wv@cg3_phone_top_5@v}{94.1}
\@namedef{wv@cg3_phone_top_5@ci}{84.1 to 98.0}
\@namedef{wv@cg3_phone_top_5@lo}{84.1}
\@namedef{wv@cg3_phone_top_5@hi}{98.0}
\@namedef{wv@cg3_top_1_gap@v}{4.6}
\@namedef{wv@cg3_top_5_gap@v}{3.1}
\@namedef{wv@cg3_unknown_median_references@v}{700.0}
\@namedef{wv@cg3_unknown_queries@v}{75}
\@namedef{wv@cg3_unknown_top_1@v}{90.7}
\@namedef{wv@cg3_unknown_top_1@ci}{82.0 to 95.4}
\@namedef{wv@cg3_unknown_top_1@lo}{82.0}
\@namedef{wv@cg3_unknown_top_1@hi}{95.4}
\@namedef{wv@cg3_unknown_top_5@v}{92.0}
\@namedef{wv@cg3_unknown_top_5@ci}{83.6 to 96.3}
\@namedef{wv@cg3_unknown_top_5@lo}{83.6}
\@namedef{wv@cg3_unknown_top_5@hi}{96.3}
\@namedef{wv@cgs_camera_median_references@v}{600.0}
\@namedef{wv@cgs_camera_queries@v}{1565}
\@namedef{wv@cgs_camera_top_1@v}{91.3}
\@namedef{wv@cgs_camera_top_1@ci}{89.8 to 92.6}
\@namedef{wv@cgs_camera_top_1@lo}{89.8}
\@namedef{wv@cgs_camera_top_1@hi}{92.6}
\@namedef{wv@cgs_camera_top_5@v}{95.0}
\@namedef{wv@cgs_camera_top_5@ci}{93.8 to 96.0}
\@namedef{wv@cgs_camera_top_5@lo}{93.8}
\@namedef{wv@cgs_camera_top_5@hi}{96.0}
\@namedef{wv@cgs_phone_median_references@v}{700.0}
\@namedef{wv@cgs_phone_queries@v}{51}
\@namedef{wv@cgs_phone_top_1@v}{86.3}
\@namedef{wv@cgs_phone_top_1@ci}{74.3 to 93.2}
\@namedef{wv@cgs_phone_top_1@lo}{74.3}
\@namedef{wv@cgs_phone_top_1@hi}{93.2}
\@namedef{wv@cgs_phone_top_5@v}{90.2}
\@namedef{wv@cgs_phone_top_5@ci}{79.0 to 95.7}
\@namedef{wv@cgs_phone_top_5@lo}{79.0}
\@namedef{wv@cgs_phone_top_5@hi}{95.7}
\@namedef{wv@cgs_top_1_gap@v}{5.0}
\@namedef{wv@cgs_top_5_gap@v}{4.8}
\@namedef{wv@cgs_unknown_median_references@v}{700.0}
\@namedef{wv@cgs_unknown_queries@v}{75}
\@namedef{wv@cgs_unknown_top_1@v}{92.0}
\@namedef{wv@cgs_unknown_top_1@ci}{83.6 to 96.3}
\@namedef{wv@cgs_unknown_top_1@lo}{83.6}
\@namedef{wv@cgs_unknown_top_1@hi}{96.3}
\@namedef{wv@cgs_unknown_top_5@v}{92.0}
\@namedef{wv@cgs_unknown_top_5@ci}{83.6 to 96.3}
\@namedef{wv@cgs_unknown_top_5@lo}{83.6}
\@namedef{wv@cgs_unknown_top_5@hi}{96.3}
\@namedef{wv@r2_cv_gate_disk-lightglue_0_top_1@v}{81.8}
\@namedef{wv@r2_cv_gate_disk-lightglue_0_top_1@ci}{78.3 to 85.2}
\@namedef{wv@r2_cv_gate_disk-lightglue_0_top_1@lo}{78.3}
\@namedef{wv@r2_cv_gate_disk-lightglue_0_top_1@hi}{85.2}
\@namedef{wv@r2_cv_gate_disk-lightglue_100_top_1@v}{84.4}
\@namedef{wv@r2_cv_gate_disk-lightglue_100_top_1@ci}{80.8 to 87.6}
\@namedef{wv@r2_cv_gate_disk-lightglue_100_top_1@lo}{80.8}
\@namedef{wv@r2_cv_gate_disk-lightglue_100_top_1@hi}{87.6}
\@namedef{wv@r2_cv_gate_disk-lightglue_10_top_1@v}{82.9}
\@namedef{wv@r2_cv_gate_disk-lightglue_10_top_1@ci}{79.3 to 86.2}
\@namedef{wv@r2_cv_gate_disk-lightglue_10_top_1@lo}{79.3}
\@namedef{wv@r2_cv_gate_disk-lightglue_10_top_1@hi}{86.2}
\@namedef{wv@r2_cv_gate_disk-lightglue_20_top_1@v}{83.9}
\@namedef{wv@r2_cv_gate_disk-lightglue_20_top_1@ci}{80.4 to 87.1}
\@namedef{wv@r2_cv_gate_disk-lightglue_20_top_1@lo}{80.4}
\@namedef{wv@r2_cv_gate_disk-lightglue_20_top_1@hi}{87.1}
\@namedef{wv@r2_cv_gate_disk-lightglue_30_top_1@v}{84.4}
\@namedef{wv@r2_cv_gate_disk-lightglue_30_top_1@ci}{81.1 to 87.7}
\@namedef{wv@r2_cv_gate_disk-lightglue_30_top_1@lo}{81.1}
\@namedef{wv@r2_cv_gate_disk-lightglue_30_top_1@hi}{87.7}
\@namedef{wv@r2_cv_gate_disk-lightglue_50_top_1@v}{84.4}
\@namedef{wv@r2_cv_gate_disk-lightglue_50_top_1@ci}{80.7 to 87.7}
\@namedef{wv@r2_cv_gate_disk-lightglue_50_top_1@lo}{80.7}
\@namedef{wv@r2_cv_gate_disk-lightglue_50_top_1@hi}{87.7}
\@namedef{wv@r2_cv_gate_disk-lightglue_5_top_1@v}{82.4}
\@namedef{wv@r2_cv_gate_disk-lightglue_5_top_1@ci}{78.8 to 85.7}
\@namedef{wv@r2_cv_gate_disk-lightglue_5_top_1@lo}{78.8}
\@namedef{wv@r2_cv_gate_disk-lightglue_5_top_1@hi}{85.7}
\@namedef{wv@r2_cv_gate_disk-lightglue_75_top_1@v}{84.4}
\@namedef{wv@r2_cv_gate_disk-lightglue_75_top_1@ci}{80.9 to 87.6}
\@namedef{wv@r2_cv_gate_disk-lightglue_75_top_1@lo}{80.9}
\@namedef{wv@r2_cv_gate_disk-lightglue_75_top_1@hi}{87.6}
\@namedef{wv@r2_cv_gate_loftr_0_top_1@v}{81.8}
\@namedef{wv@r2_cv_gate_loftr_0_top_1@ci}{78.2 to 85.3}
\@namedef{wv@r2_cv_gate_loftr_0_top_1@lo}{78.2}
\@namedef{wv@r2_cv_gate_loftr_0_top_1@hi}{85.3}
\@namedef{wv@r2_cv_gate_loftr_100_top_1@v}{85.5}
\@namedef{wv@r2_cv_gate_loftr_100_top_1@ci}{82.2 to 88.5}
\@namedef{wv@r2_cv_gate_loftr_100_top_1@lo}{82.2}
\@namedef{wv@r2_cv_gate_loftr_100_top_1@hi}{88.5}
\@namedef{wv@r2_cv_gate_loftr_10_top_1@v}{83.3}
\@namedef{wv@r2_cv_gate_loftr_10_top_1@ci}{79.9 to 86.5}
\@namedef{wv@r2_cv_gate_loftr_10_top_1@lo}{79.9}
\@namedef{wv@r2_cv_gate_loftr_10_top_1@hi}{86.5}
\@namedef{wv@r2_cv_gate_loftr_20_top_1@v}{84.5}
\@namedef{wv@r2_cv_gate_loftr_20_top_1@ci}{81.2 to 87.6}
\@namedef{wv@r2_cv_gate_loftr_20_top_1@lo}{81.2}
\@namedef{wv@r2_cv_gate_loftr_20_top_1@hi}{87.6}
\@namedef{wv@r2_cv_gate_loftr_30_top_1@v}{85.3}
\@namedef{wv@r2_cv_gate_loftr_30_top_1@ci}{82.1 to 88.3}
\@namedef{wv@r2_cv_gate_loftr_30_top_1@lo}{82.1}
\@namedef{wv@r2_cv_gate_loftr_30_top_1@hi}{88.3}
\@namedef{wv@r2_cv_gate_loftr_50_top_1@v}{85.5}
\@namedef{wv@r2_cv_gate_loftr_50_top_1@ci}{82.2 to 88.5}
\@namedef{wv@r2_cv_gate_loftr_50_top_1@lo}{82.2}
\@namedef{wv@r2_cv_gate_loftr_50_top_1@hi}{88.5}
\@namedef{wv@r2_cv_gate_loftr_5_top_1@v}{82.7}
\@namedef{wv@r2_cv_gate_loftr_5_top_1@ci}{79.1 to 85.9}
\@namedef{wv@r2_cv_gate_loftr_5_top_1@lo}{79.1}
\@namedef{wv@r2_cv_gate_loftr_5_top_1@hi}{85.9}
\@namedef{wv@r2_cv_gate_loftr_75_top_1@v}{85.5}
\@namedef{wv@r2_cv_gate_loftr_75_top_1@ci}{82.2 to 88.5}
\@namedef{wv@r2_cv_gate_loftr_75_top_1@lo}{82.2}
\@namedef{wv@r2_cv_gate_loftr_75_top_1@hi}{88.5}
\@namedef{wv@r2_cv_gate_sift_0_top_1@v}{81.8}
\@namedef{wv@r2_cv_gate_sift_0_top_1@ci}{78.2 to 85.2}
\@namedef{wv@r2_cv_gate_sift_0_top_1@lo}{78.2}
\@namedef{wv@r2_cv_gate_sift_0_top_1@hi}{85.2}
\@namedef{wv@r2_cv_gate_sift_100_top_1@v}{82.1}
\@namedef{wv@r2_cv_gate_sift_100_top_1@ci}{78.5 to 85.4}
\@namedef{wv@r2_cv_gate_sift_100_top_1@lo}{78.5}
\@namedef{wv@r2_cv_gate_sift_100_top_1@hi}{85.4}
\@namedef{wv@r2_cv_gate_sift_10_top_1@v}{81.9}
\@namedef{wv@r2_cv_gate_sift_10_top_1@ci}{78.4 to 85.2}
\@namedef{wv@r2_cv_gate_sift_10_top_1@lo}{78.4}
\@namedef{wv@r2_cv_gate_sift_10_top_1@hi}{85.2}
\@namedef{wv@r2_cv_gate_sift_20_top_1@v}{82.1}
\@namedef{wv@r2_cv_gate_sift_20_top_1@ci}{78.5 to 85.4}
\@namedef{wv@r2_cv_gate_sift_20_top_1@lo}{78.5}
\@namedef{wv@r2_cv_gate_sift_20_top_1@hi}{85.4}
\@namedef{wv@r2_cv_gate_sift_30_top_1@v}{82.1}
\@namedef{wv@r2_cv_gate_sift_30_top_1@ci}{78.6 to 85.5}
\@namedef{wv@r2_cv_gate_sift_30_top_1@lo}{78.6}
\@namedef{wv@r2_cv_gate_sift_30_top_1@hi}{85.5}
\@namedef{wv@r2_cv_gate_sift_50_top_1@v}{82.1}
\@namedef{wv@r2_cv_gate_sift_50_top_1@ci}{78.6 to 85.3}
\@namedef{wv@r2_cv_gate_sift_50_top_1@lo}{78.6}
\@namedef{wv@r2_cv_gate_sift_50_top_1@hi}{85.3}
\@namedef{wv@r2_cv_gate_sift_5_top_1@v}{81.9}
\@namedef{wv@r2_cv_gate_sift_5_top_1@ci}{78.4 to 85.2}
\@namedef{wv@r2_cv_gate_sift_5_top_1@lo}{78.4}
\@namedef{wv@r2_cv_gate_sift_5_top_1@hi}{85.2}
\@namedef{wv@r2_cv_gate_sift_75_top_1@v}{82.1}
\@namedef{wv@r2_cv_gate_sift_75_top_1@ci}{78.6 to 85.3}
\@namedef{wv@r2_cv_gate_sift_75_top_1@lo}{78.6}
\@namedef{wv@r2_cv_gate_sift_75_top_1@hi}{85.3}
\@namedef{wv@r2_dinov2_mr_disjoint_cosine_top_1@v}{81.8}
\@namedef{wv@r2_dinov2_mr_disjoint_cosine_top_1@ci}{78.2 to 85.2}
\@namedef{wv@r2_dinov2_mr_disjoint_cosine_top_1@lo}{78.2}
\@namedef{wv@r2_dinov2_mr_disjoint_cosine_top_1@hi}{85.2}
\@namedef{wv@r2_dinov2_mr_disjoint_cosine_top_10@v}{90.8}
\@namedef{wv@r2_dinov2_mr_disjoint_cosine_top_10@ci}{87.9 to 93.3}
\@namedef{wv@r2_dinov2_mr_disjoint_cosine_top_10@lo}{87.9}
\@namedef{wv@r2_dinov2_mr_disjoint_cosine_top_10@hi}{93.3}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_top_1@v}{81.2}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_top_1@ci}{77.1 to 84.9}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_top_1@lo}{77.1}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_top_1@hi}{84.9}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_top_10@v}{91.3}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_top_10@ci}{88.3 to 93.8}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_top_10@lo}{88.3}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_top_10@hi}{93.8}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_10_gain@v}{0.5}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_10_gain@ci}{$-$1.0 to 2.0}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_10_gain@lo}{$-$1.0}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_10_gain@hi}{2.0}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_10_losses@v}{25}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_10_wins@v}{31}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_1_gain@v}{$-$0.7}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_1_gain@ci}{$-$3.0 to 1.6}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_1_gain@lo}{$-$3.0}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_1_gain@hi}{1.6}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_1_losses@v}{67}
\@namedef{wv@r2_dinov2_mr_disjoint_grid14_vs_cosine_top_1_wins@v}{59}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_top_1@v}{79.9}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_top_1@ci}{75.6 to 83.8}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_top_1@lo}{75.6}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_top_1@hi}{83.8}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_top_10@v}{90.8}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_top_10@ci}{87.9 to 93.4}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_top_10@lo}{87.9}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_top_10@hi}{93.4}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_10_gain@v}{0.0}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_10_gain@ci}{$-$1.4 to 1.4}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_10_gain@lo}{$-$1.4}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_10_gain@hi}{1.4}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_10_losses@v}{28}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_10_wins@v}{28}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_1_gain@v}{$-$2.0}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_1_gain@ci}{$-$4.4 to 0.4}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_1_gain@lo}{$-$4.4}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_1_gain@hi}{0.4}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_1_losses@v}{70}
\@namedef{wv@r2_dinov2_mr_disjoint_grid5_vs_cosine_top_1_wins@v}{47}
\@namedef{wv@r2_dinov2_mr_disjoint_queries@v}{1157}
\@namedef{wv@r2_dinov2_mr_full_cosine_top_1@v}{93.1}
\@namedef{wv@r2_dinov2_mr_full_cosine_top_1@ci}{91.8 to 94.4}
\@namedef{wv@r2_dinov2_mr_full_cosine_top_1@lo}{91.8}
\@namedef{wv@r2_dinov2_mr_full_cosine_top_1@hi}{94.4}
\@namedef{wv@r2_dinov2_mr_full_cosine_top_10@v}{96.2}
\@namedef{wv@r2_dinov2_mr_full_cosine_top_10@ci}{95.2 to 97.1}
\@namedef{wv@r2_dinov2_mr_full_cosine_top_10@lo}{95.2}
\@namedef{wv@r2_dinov2_mr_full_cosine_top_10@hi}{97.1}
\@namedef{wv@r2_dinov2_mr_full_grid14_top_1@v}{93.8}
\@namedef{wv@r2_dinov2_mr_full_grid14_top_1@ci}{92.5 to 95.0}
\@namedef{wv@r2_dinov2_mr_full_grid14_top_1@lo}{92.5}
\@namedef{wv@r2_dinov2_mr_full_grid14_top_1@hi}{95.0}
\@namedef{wv@r2_dinov2_mr_full_grid14_top_10@v}{97.0}
\@namedef{wv@r2_dinov2_mr_full_grid14_top_10@ci}{96.1 to 97.8}
\@namedef{wv@r2_dinov2_mr_full_grid14_top_10@lo}{96.1}
\@namedef{wv@r2_dinov2_mr_full_grid14_top_10@hi}{97.8}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_10_gain@v}{0.8}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_10_gain@ci}{0.1 to 1.4}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_10_gain@lo}{0.1}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_10_gain@hi}{1.4}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_10_losses@v}{10}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_10_wins@v}{23}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_1_gain@v}{0.7}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_1_gain@ci}{$-$0.3 to 1.6}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_1_gain@lo}{$-$0.3}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_1_gain@hi}{1.6}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_1_losses@v}{32}
\@namedef{wv@r2_dinov2_mr_full_grid14_vs_cosine_top_1_wins@v}{43}
\@namedef{wv@r2_dinov2_mr_full_grid5_top_1@v}{93.1}
\@namedef{wv@r2_dinov2_mr_full_grid5_top_1@ci}{91.8 to 94.4}
\@namedef{wv@r2_dinov2_mr_full_grid5_top_1@lo}{91.8}
\@namedef{wv@r2_dinov2_mr_full_grid5_top_1@hi}{94.4}
\@namedef{wv@r2_dinov2_mr_full_grid5_top_10@v}{96.9}
\@namedef{wv@r2_dinov2_mr_full_grid5_top_10@ci}{96.1 to 97.7}
\@namedef{wv@r2_dinov2_mr_full_grid5_top_10@lo}{96.1}
\@namedef{wv@r2_dinov2_mr_full_grid5_top_10@hi}{97.7}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_10_gain@v}{0.7}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_10_gain@ci}{0.1 to 1.3}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_10_gain@lo}{0.1}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_10_gain@hi}{1.3}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_10_losses@v}{8}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_10_wins@v}{20}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_1_gain@v}{0.0}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_1_gain@ci}{$-$0.9 to 0.9}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_1_gain@lo}{$-$0.9}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_1_gain@hi}{0.9}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_1_losses@v}{37}
\@namedef{wv@r2_dinov2_mr_full_grid5_vs_cosine_top_1_wins@v}{37}
\@namedef{wv@r2_dinov2_mr_full_queries@v}{1691}
\@namedef{wv@r2_dinov2_strata_1_queries@v}{207}
\@namedef{wv@r2_dinov2_strata_1_statues@v}{66}
\@namedef{wv@r2_dinov2_strata_1_top_1@v}{60.4}
\@namedef{wv@r2_dinov2_strata_1_top_1@ci}{51.1 to 70.1}
\@namedef{wv@r2_dinov2_strata_1_top_1@lo}{51.1}
\@namedef{wv@r2_dinov2_strata_1_top_1@hi}{70.1}
\@namedef{wv@r2_dinov2_strata_2_queries@v}{207}
\@namedef{wv@r2_dinov2_strata_2_statues@v}{84}
\@namedef{wv@r2_dinov2_strata_2_top_1@v}{78.3}
\@namedef{wv@r2_dinov2_strata_2_top_1@ci}{71.1 to 85.4}
\@namedef{wv@r2_dinov2_strata_2_top_1@lo}{71.1}
\@namedef{wv@r2_dinov2_strata_2_top_1@hi}{85.4}
\@namedef{wv@r2_dinov2_strata_3to5_queries@v}{347}
\@namedef{wv@r2_dinov2_strata_3to5_statues@v}{99}
\@namedef{wv@r2_dinov2_strata_3to5_top_1@v}{85.0}
\@namedef{wv@r2_dinov2_strata_3to5_top_1@ci}{80.4 to 89.6}
\@namedef{wv@r2_dinov2_strata_3to5_top_1@lo}{80.4}
\@namedef{wv@r2_dinov2_strata_3to5_top_1@hi}{89.6}
\@namedef{wv@r2_dinov2_strata_6plus_queries@v}{396}
\@namedef{wv@r2_dinov2_strata_6plus_statues@v}{67}
\@namedef{wv@r2_dinov2_strata_6plus_top_1@v}{92.2}
\@namedef{wv@r2_dinov2_strata_6plus_top_1@ci}{89.3 to 94.9}
\@namedef{wv@r2_dinov2_strata_6plus_top_1@lo}{89.3}
\@namedef{wv@r2_dinov2_strata_6plus_top_1@hi}{94.9}
\@namedef{wv@r2_dinov3_mr_disjoint_cosine_top_1@v}{85.2}
\@namedef{wv@r2_dinov3_mr_disjoint_cosine_top_1@ci}{81.9 to 88.3}
\@namedef{wv@r2_dinov3_mr_disjoint_cosine_top_1@lo}{81.9}
\@namedef{wv@r2_dinov3_mr_disjoint_cosine_top_1@hi}{88.3}
\@namedef{wv@r2_dinov3_mr_disjoint_cosine_top_10@v}{92.8}
\@namedef{wv@r2_dinov3_mr_disjoint_cosine_top_10@ci}{90.4 to 95.0}
\@namedef{wv@r2_dinov3_mr_disjoint_cosine_top_10@lo}{90.4}
\@namedef{wv@r2_dinov3_mr_disjoint_cosine_top_10@hi}{95.0}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_top_1@v}{82.6}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_top_1@ci}{78.8 to 86.2}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_top_1@lo}{78.8}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_top_1@hi}{86.2}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_top_10@v}{91.9}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_top_10@ci}{88.9 to 94.5}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_top_10@lo}{88.9}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_top_10@hi}{94.5}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_10_gain@v}{$-$1.0}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_10_gain@ci}{$-$3.1 to 0.9}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_10_gain@lo}{$-$3.1}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_10_gain@hi}{0.9}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_10_losses@v}{35}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_10_wins@v}{24}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_1_gain@v}{$-$2.6}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_1_gain@ci}{$-$5.2 to $-$0.1}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_1_gain@lo}{$-$5.2}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_1_gain@hi}{$-$0.1}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_1_losses@v}{74}
\@namedef{wv@r2_dinov3_mr_disjoint_grid14_vs_cosine_top_1_wins@v}{44}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_top_1@v}{83.3}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_top_1@ci}{79.5 to 86.9}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_top_1@lo}{79.5}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_top_1@hi}{86.9}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_top_10@v}{92.0}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_top_10@ci}{89.2 to 94.6}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_top_10@lo}{89.2}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_top_10@hi}{94.6}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_10_gain@v}{$-$0.8}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_10_gain@ci}{$-$2.5 to 0.8}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_10_gain@lo}{$-$2.5}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_10_gain@hi}{0.8}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_10_losses@v}{29}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_10_wins@v}{20}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_1_gain@v}{$-$1.9}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_1_gain@ci}{$-$4.1 to 0.2}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_1_gain@lo}{$-$4.1}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_1_gain@hi}{0.2}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_1_losses@v}{59}
\@namedef{wv@r2_dinov3_mr_disjoint_grid5_vs_cosine_top_1_wins@v}{37}
\@namedef{wv@r2_dinov3_mr_disjoint_queries@v}{1157}
\@namedef{wv@r2_dinov3_mr_full_cosine_top_1@v}{94.4}
\@namedef{wv@r2_dinov3_mr_full_cosine_top_1@ci}{93.1 to 95.6}
\@namedef{wv@r2_dinov3_mr_full_cosine_top_1@lo}{93.1}
\@namedef{wv@r2_dinov3_mr_full_cosine_top_1@hi}{95.6}
\@namedef{wv@r2_dinov3_mr_full_cosine_top_10@v}{97.5}
\@namedef{wv@r2_dinov3_mr_full_cosine_top_10@ci}{96.7 to 98.3}
\@namedef{wv@r2_dinov3_mr_full_cosine_top_10@lo}{96.7}
\@namedef{wv@r2_dinov3_mr_full_cosine_top_10@hi}{98.3}
\@namedef{wv@r2_dinov3_mr_full_grid14_top_1@v}{94.4}
\@namedef{wv@r2_dinov3_mr_full_grid14_top_1@ci}{93.2 to 95.6}
\@namedef{wv@r2_dinov3_mr_full_grid14_top_1@lo}{93.2}
\@namedef{wv@r2_dinov3_mr_full_grid14_top_1@hi}{95.6}
\@namedef{wv@r2_dinov3_mr_full_grid14_top_10@v}{97.4}
\@namedef{wv@r2_dinov3_mr_full_grid14_top_10@ci}{96.5 to 98.2}
\@namedef{wv@r2_dinov3_mr_full_grid14_top_10@lo}{96.5}
\@namedef{wv@r2_dinov3_mr_full_grid14_top_10@hi}{98.2}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_10_gain@v}{$-$0.1}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_10_gain@ci}{$-$0.7 to 0.5}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_10_gain@lo}{$-$0.7}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_10_gain@hi}{0.5}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_10_losses@v}{13}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_10_wins@v}{11}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_1_gain@v}{0.0}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_1_gain@ci}{$-$0.8 to 0.8}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_1_gain@lo}{$-$0.8}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_1_gain@hi}{0.8}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_1_losses@v}{23}
\@namedef{wv@r2_dinov3_mr_full_grid14_vs_cosine_top_1_wins@v}{23}
\@namedef{wv@r2_dinov3_mr_full_grid5_top_1@v}{94.5}
\@namedef{wv@r2_dinov3_mr_full_grid5_top_1@ci}{93.2 to 95.7}
\@namedef{wv@r2_dinov3_mr_full_grid5_top_1@lo}{93.2}
\@namedef{wv@r2_dinov3_mr_full_grid5_top_1@hi}{95.7}
\@namedef{wv@r2_dinov3_mr_full_grid5_top_10@v}{97.7}
\@namedef{wv@r2_dinov3_mr_full_grid5_top_10@ci}{96.9 to 98.4}
\@namedef{wv@r2_dinov3_mr_full_grid5_top_10@lo}{96.9}
\@namedef{wv@r2_dinov3_mr_full_grid5_top_10@hi}{98.4}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_10_gain@v}{0.2}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_10_gain@ci}{$-$0.3 to 0.7}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_10_gain@lo}{$-$0.3}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_10_gain@hi}{0.7}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_10_losses@v}{7}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_10_wins@v}{10}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_1_gain@v}{0.1}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_1_gain@ci}{$-$0.7 to 0.8}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_1_gain@lo}{$-$0.7}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_1_gain@hi}{0.8}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_1_losses@v}{20}
\@namedef{wv@r2_dinov3_mr_full_grid5_vs_cosine_top_1_wins@v}{21}
\@namedef{wv@r2_dinov3_mr_full_queries@v}{1691}
\@namedef{wv@r2_dinov3_strata_1_queries@v}{207}
\@namedef{wv@r2_dinov3_strata_1_statues@v}{66}
\@namedef{wv@r2_dinov3_strata_1_top_1@v}{69.6}
\@namedef{wv@r2_dinov3_strata_1_top_1@ci}{60.6 to 78.9}
\@namedef{wv@r2_dinov3_strata_1_top_1@lo}{60.6}
\@namedef{wv@r2_dinov3_strata_1_top_1@hi}{78.9}
\@namedef{wv@r2_dinov3_strata_2_queries@v}{207}
\@namedef{wv@r2_dinov3_strata_2_statues@v}{84}
\@namedef{wv@r2_dinov3_strata_2_top_1@v}{81.2}
\@namedef{wv@r2_dinov3_strata_2_top_1@ci}{74.8 to 87.4}
\@namedef{wv@r2_dinov3_strata_2_top_1@lo}{74.8}
\@namedef{wv@r2_dinov3_strata_2_top_1@hi}{87.4}
\@namedef{wv@r2_dinov3_strata_3to5_queries@v}{347}
\@namedef{wv@r2_dinov3_strata_3to5_statues@v}{99}
\@namedef{wv@r2_dinov3_strata_3to5_top_1@v}{88.2}
\@namedef{wv@r2_dinov3_strata_3to5_top_1@ci}{83.2 to 92.4}
\@namedef{wv@r2_dinov3_strata_3to5_top_1@lo}{83.2}
\@namedef{wv@r2_dinov3_strata_3to5_top_1@hi}{92.4}
\@namedef{wv@r2_dinov3_strata_6plus_queries@v}{396}
\@namedef{wv@r2_dinov3_strata_6plus_statues@v}{67}
\@namedef{wv@r2_dinov3_strata_6plus_top_1@v}{92.9}
\@namedef{wv@r2_dinov3_strata_6plus_top_1@ci}{89.7 to 95.7}
\@namedef{wv@r2_dinov3_strata_6plus_top_1@lo}{89.7}
\@namedef{wv@r2_dinov3_strata_6plus_top_1@hi}{95.7}
\@namedef{wv@v3_cv_cosine_top_1@v}{85.2}
\@namedef{wv@v3_cv_cosine_top_1@ci}{83.1 to 87.1}
\@namedef{wv@v3_cv_cosine_top_1@lo}{83.1}
\@namedef{wv@v3_cv_cosine_top_1@hi}{87.1}
\@namedef{wv@v3_cv_cosine_top_5@v}{90.9}
\@namedef{wv@v3_cv_cosine_top_5@ci}{89.1 to 92.4}
\@namedef{wv@v3_cv_cosine_top_5@lo}{89.1}
\@namedef{wv@v3_cv_cosine_top_5@hi}{92.4}
\@namedef{wv@v3_cv_disk-lightglue_top_1@v}{87.2}
\@namedef{wv@v3_cv_disk-lightglue_top_1@ci}{85.2 to 89.0}
\@namedef{wv@v3_cv_disk-lightglue_top_1@lo}{85.2}
\@namedef{wv@v3_cv_disk-lightglue_top_1@hi}{89.0}
\@namedef{wv@v3_cv_disk-lightglue_top_5@v}{91.7}
\@namedef{wv@v3_cv_disk-lightglue_top_5@ci}{90.0 to 93.2}
\@namedef{wv@v3_cv_disk-lightglue_top_5@lo}{90.0}
\@namedef{wv@v3_cv_disk-lightglue_top_5@hi}{93.2}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_1_gain@v}{2.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_1_gain@ci}{1.0 to 3.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_1_gain@lo}{1.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_1_gain@hi}{3.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_1_losses@v}{7}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_1_p_value@v}{$1.9\times10^{-4}$}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_1_wins@v}{30}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_5_gain@v}{0.8}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_5_gain@ci}{0.3 to 1.4}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_5_gain@lo}{0.3}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_5_gain@hi}{1.4}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_5_losses@v}{1}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_5_p_value@v}{0.012}
\@namedef{wv@v3_cv_disk-lightglue_vs_cosine_top_5_wins@v}{10}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_1_gain@v}{2.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_1_gain@ci}{1.0 to 3.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_1_gain@lo}{1.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_1_gain@hi}{3.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_1_losses@v}{6}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_1_p_value@v}{$1.2\times10^{-4}$}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_1_wins@v}{29}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_5_gain@v}{0.5}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_5_gain@ci}{0.0 to 1.1}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_5_gain@lo}{0.0}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_5_gain@hi}{1.1}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_5_losses@v}{2}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_5_p_value@v}{0.11}
\@namedef{wv@v3_cv_disk-lightglue_vs_sift_top_5_wins@v}{8}
\@namedef{wv@v3_cv_loftr_top_1@v}{86.7}
\@namedef{wv@v3_cv_loftr_top_1@ci}{84.6 to 88.5}
\@namedef{wv@v3_cv_loftr_top_1@lo}{84.6}
\@namedef{wv@v3_cv_loftr_top_1@hi}{88.5}
\@namedef{wv@v3_cv_loftr_top_5@v}{91.9}
\@namedef{wv@v3_cv_loftr_top_5@ci}{90.2 to 93.3}
\@namedef{wv@v3_cv_loftr_top_5@lo}{90.2}
\@namedef{wv@v3_cv_loftr_top_5@hi}{93.3}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_1_gain@v}{1.5}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_1_gain@ci}{0.3 to 2.5}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_1_gain@lo}{0.3}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_1_gain@hi}{2.5}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_1_losses@v}{12}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_1_p_value@v}{0.012}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_1_wins@v}{29}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_5_gain@v}{1.0}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_5_gain@ci}{0.3 to 1.6}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_5_gain@lo}{0.3}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_5_gain@hi}{1.6}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_5_losses@v}{2}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_5_p_value@v}{0.0074}
\@namedef{wv@v3_cv_loftr_vs_cosine_top_5_wins@v}{13}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_1_gain@v}{$-$0.5}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_1_gain@ci}{$-$1.5 to 0.3}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_1_gain@lo}{$-$1.5}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_1_gain@hi}{0.3}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_1_losses@v}{17}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_1_p_value@v}{0.34}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_1_wins@v}{11}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_5_gain@v}{0.2}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_5_gain@ci}{$-$0.4 to 0.7}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_5_gain@lo}{$-$0.4}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_5_gain@hi}{0.7}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_5_losses@v}{3}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_5_p_value@v}{0.73}
\@namedef{wv@v3_cv_loftr_vs_disk-lightglue_top_5_wins@v}{5}
\@namedef{wv@v3_cv_loftr_vs_sift_top_1_gain@v}{1.5}
\@namedef{wv@v3_cv_loftr_vs_sift_top_1_gain@ci}{0.3 to 2.6}
\@namedef{wv@v3_cv_loftr_vs_sift_top_1_gain@lo}{0.3}
\@namedef{wv@v3_cv_loftr_vs_sift_top_1_gain@hi}{2.6}
\@namedef{wv@v3_cv_loftr_vs_sift_top_1_losses@v}{11}
\@namedef{wv@v3_cv_loftr_vs_sift_top_1_p_value@v}{0.0095}
\@namedef{wv@v3_cv_loftr_vs_sift_top_1_wins@v}{28}
\@namedef{wv@v3_cv_loftr_vs_sift_top_5_gain@v}{0.7}
\@namedef{wv@v3_cv_loftr_vs_sift_top_5_gain@ci}{0.1 to 1.3}
\@namedef{wv@v3_cv_loftr_vs_sift_top_5_gain@lo}{0.1}
\@namedef{wv@v3_cv_loftr_vs_sift_top_5_gain@hi}{1.3}
\@namedef{wv@v3_cv_loftr_vs_sift_top_5_losses@v}{3}
\@namedef{wv@v3_cv_loftr_vs_sift_top_5_p_value@v}{0.057}
\@namedef{wv@v3_cv_loftr_vs_sift_top_5_wins@v}{11}
\@namedef{wv@v3_cv_queries@v}{1157}
\@namedef{wv@v3_cv_sift_top_1@v}{85.2}
\@namedef{wv@v3_cv_sift_top_1@ci}{83.1 to 87.1}
\@namedef{wv@v3_cv_sift_top_1@lo}{83.1}
\@namedef{wv@v3_cv_sift_top_1@hi}{87.1}
\@namedef{wv@v3_cv_sift_top_5@v}{91.2}
\@namedef{wv@v3_cv_sift_top_5@ci}{89.4 to 92.7}
\@namedef{wv@v3_cv_sift_top_5@lo}{89.4}
\@namedef{wv@v3_cv_sift_top_5@hi}{92.7}
\@namedef{wv@v3_cv_sift_vs_cosine_top_1_gain@v}{0.0}
\@namedef{wv@v3_cv_sift_vs_cosine_top_1_gain@ci}{$-$0.5 to 0.5}
\@namedef{wv@v3_cv_sift_vs_cosine_top_1_gain@lo}{$-$0.5}
\@namedef{wv@v3_cv_sift_vs_cosine_top_1_gain@hi}{0.5}
\@namedef{wv@v3_cv_sift_vs_cosine_top_1_losses@v}{5}
\@namedef{wv@v3_cv_sift_vs_cosine_top_1_p_value@v}{1}
\@namedef{wv@v3_cv_sift_vs_cosine_top_1_wins@v}{5}
\@namedef{wv@v3_cv_sift_vs_cosine_top_5_gain@v}{0.3}
\@namedef{wv@v3_cv_sift_vs_cosine_top_5_gain@ci}{0.0 to 0.6}
\@namedef{wv@v3_cv_sift_vs_cosine_top_5_gain@lo}{0.0}
\@namedef{wv@v3_cv_sift_vs_cosine_top_5_gain@hi}{0.6}
\@namedef{wv@v3_cv_sift_vs_cosine_top_5_losses@v}{0}
\@namedef{wv@v3_cv_sift_vs_cosine_top_5_p_value@v}{0.25}
\@namedef{wv@v3_cv_sift_vs_cosine_top_5_wins@v}{3}
\@namedef{wv@v3_cv_statues@v}{181}
\makeatother


==> generated/family-numbers.tex <==
\makeatletter
\@namedef{wv@fam_aimv2_cosine_false_acceptance_90@v}{42.6}
\@namedef{wv@fam_aimv2_geo_minus_random_pool_10@v}{$-$1.0}
\@namedef{wv@fam_aimv2_geo_minus_random_pool_10@ci}{$-$1.7 to $-$0.3}
\@namedef{wv@fam_aimv2_geo_minus_random_pool_10@lo}{$-$1.7}
\@namedef{wv@fam_aimv2_geo_minus_random_pool_10@hi}{$-$0.3}
\@namedef{wv@fam_aimv2_mrr@v}{0.923}
\@namedef{wv@fam_aimv2_photographer_attributable@v}{5.5}
\@namedef{wv@fam_aimv2_photographer_attributable@ci}{3.2 to 7.7}
\@namedef{wv@fam_aimv2_photographer_attributable@lo}{3.2}
\@namedef{wv@fam_aimv2_photographer_attributable@hi}{7.7}
\@namedef{wv@fam_aimv2_points_per_doubling@v}{$-$1.1}
\@namedef{wv@fam_aimv2_points_per_doubling@ci}{$-$1.3 to $-$0.9}
\@namedef{wv@fam_aimv2_points_per_doubling@lo}{$-$1.3}
\@namedef{wv@fam_aimv2_points_per_doubling@hi}{$-$0.9}
\@namedef{wv@fam_aimv2_reject_cosine_auroc@v}{0.895}
\@namedef{wv@fam_aimv2_reject_cosine_auroc@ci}{0.882 to 0.907}
\@namedef{wv@fam_aimv2_reject_cosine_auroc@lo}{0.882}
\@namedef{wv@fam_aimv2_reject_cosine_auroc@hi}{0.907}
\@namedef{wv@fam_aimv2_reject_margin_auroc@v}{0.922}
\@namedef{wv@fam_aimv2_reject_margin_auroc@ci}{0.911 to 0.933}
\@namedef{wv@fam_aimv2_reject_margin_auroc@lo}{0.911}
\@namedef{wv@fam_aimv2_reject_margin_auroc@hi}{0.933}
\@namedef{wv@fam_aimv2_reject_margin_false_acceptance_90@v}{27.8}
\@namedef{wv@fam_aimv2_top_1@v}{90.7}
\@namedef{wv@fam_aimv2_top_1@ci}{89.1 to 92.3}
\@namedef{wv@fam_aimv2_top_1@lo}{89.1}
\@namedef{wv@fam_aimv2_top_1@hi}{92.3}
\@namedef{wv@fam_aimv2_top_5@v}{94.4}
\@namedef{wv@fam_aimv2_unseen_r_at_10@v}{85.1}
\@namedef{wv@fam_aimv2_unseen_top_1@v}{74.0}
\@namedef{wv@fam_beit_cosine_false_acceptance_90@v}{82.9}
\@namedef{wv@fam_beit_geo_minus_random_pool_10@v}{$-$4.1}
\@namedef{wv@fam_beit_geo_minus_random_pool_10@ci}{$-$6.1 to $-$2.2}
\@namedef{wv@fam_beit_geo_minus_random_pool_10@lo}{$-$6.1}
\@namedef{wv@fam_beit_geo_minus_random_pool_10@hi}{$-$2.2}
\@namedef{wv@fam_beit_mrr@v}{0.612}
\@namedef{wv@fam_beit_photographer_attributable@v}{15.0}
\@namedef{wv@fam_beit_photographer_attributable@ci}{12.4 to 17.7}
\@namedef{wv@fam_beit_photographer_attributable@lo}{12.4}
\@namedef{wv@fam_beit_photographer_attributable@hi}{17.7}
\@namedef{wv@fam_beit_points_per_doubling@v}{$-$5.6}
\@namedef{wv@fam_beit_points_per_doubling@ci}{$-$6.1 to $-$5.2}
\@namedef{wv@fam_beit_points_per_doubling@lo}{$-$6.1}
\@namedef{wv@fam_beit_points_per_doubling@hi}{$-$5.2}
\@namedef{wv@fam_beit_reject_cosine_auroc@v}{0.634}
\@namedef{wv@fam_beit_reject_cosine_auroc@ci}{0.619 to 0.651}
\@namedef{wv@fam_beit_reject_cosine_auroc@lo}{0.619}
\@namedef{wv@fam_beit_reject_cosine_auroc@hi}{0.651}
\@namedef{wv@fam_beit_reject_margin_auroc@v}{0.667}
\@namedef{wv@fam_beit_reject_margin_auroc@ci}{0.646 to 0.688}
\@namedef{wv@fam_beit_reject_margin_auroc@lo}{0.646}
\@namedef{wv@fam_beit_reject_margin_auroc@hi}{0.688}
\@namedef{wv@fam_beit_reject_margin_false_acceptance_90@v}{81.2}
\@namedef{wv@fam_beit_top_1@v}{52.8}
\@namedef{wv@fam_beit_top_1@ci}{49.2 to 56.3}
\@namedef{wv@fam_beit_top_1@lo}{49.2}
\@namedef{wv@fam_beit_top_1@hi}{56.3}
\@namedef{wv@fam_beit_top_5@v}{70.1}
\@namedef{wv@fam_beit_unseen_r_at_10@v}{42.9}
\@namedef{wv@fam_beit_unseen_top_1@v}{20.7}
\@namedef{wv@fam_clip-b16_cosine_false_acceptance_90@v}{60.9}
\@namedef{wv@fam_clip-b16_geo_minus_random_pool_10@v}{$-$1.1}
\@namedef{wv@fam_clip-b16_geo_minus_random_pool_10@ci}{$-$1.8 to $-$0.4}
\@namedef{wv@fam_clip-b16_geo_minus_random_pool_10@lo}{$-$1.8}
\@namedef{wv@fam_clip-b16_geo_minus_random_pool_10@hi}{$-$0.4}
\@namedef{wv@fam_clip-b16_mrr@v}{0.900}
\@namedef{wv@fam_clip-b16_photographer_attributable@v}{10.0}
\@namedef{wv@fam_clip-b16_photographer_attributable@ci}{7.4 to 12.5}
\@namedef{wv@fam_clip-b16_photographer_attributable@lo}{7.4}
\@namedef{wv@fam_clip-b16_photographer_attributable@hi}{12.5}
\@namedef{wv@fam_clip-b16_points_per_doubling@v}{$-$1.5}
\@namedef{wv@fam_clip-b16_points_per_doubling@ci}{$-$1.7 to $-$1.2}
\@namedef{wv@fam_clip-b16_points_per_doubling@lo}{$-$1.7}
\@namedef{wv@fam_clip-b16_points_per_doubling@hi}{$-$1.2}
\@namedef{wv@fam_clip-b16_reject_cosine_auroc@v}{0.835}
\@namedef{wv@fam_clip-b16_reject_cosine_auroc@ci}{0.818 to 0.852}
\@namedef{wv@fam_clip-b16_reject_cosine_auroc@lo}{0.818}
\@namedef{wv@fam_clip-b16_reject_cosine_auroc@hi}{0.852}
\@namedef{wv@fam_clip-b16_reject_margin_auroc@v}{0.895}
\@namedef{wv@fam_clip-b16_reject_margin_auroc@ci}{0.881 to 0.908}
\@namedef{wv@fam_clip-b16_reject_margin_auroc@lo}{0.881}
\@namedef{wv@fam_clip-b16_reject_margin_auroc@hi}{0.908}
\@namedef{wv@fam_clip-b16_reject_margin_false_acceptance_90@v}{42.8}
\@namedef{wv@fam_clip-b16_top_1@v}{87.7}
\@namedef{wv@fam_clip-b16_top_1@ci}{85.9 to 89.4}
\@namedef{wv@fam_clip-b16_top_1@lo}{85.9}
\@namedef{wv@fam_clip-b16_top_1@hi}{89.4}
\@namedef{wv@fam_clip-b16_top_5@v}{92.6}
\@namedef{wv@fam_clip-b16_unseen_r_at_10@v}{79.9}
\@namedef{wv@fam_clip-b16_unseen_top_1@v}{63.6}
\@namedef{wv@fam_clip_cosine_false_acceptance_90@v}{67.4}
\@namedef{wv@fam_clip_geo_minus_random_pool_10@v}{$-$2.1}
\@namedef{wv@fam_clip_geo_minus_random_pool_10@ci}{$-$3.1 to $-$1.2}
\@namedef{wv@fam_clip_geo_minus_random_pool_10@lo}{$-$3.1}
\@namedef{wv@fam_clip_geo_minus_random_pool_10@hi}{$-$1.2}
\@namedef{wv@fam_clip_mrr@v}{0.866}
\@namedef{wv@fam_clip_photographer_attributable@v}{13.2}
\@namedef{wv@fam_clip_photographer_attributable@ci}{10.5 to 16.1}
\@namedef{wv@fam_clip_photographer_attributable@lo}{10.5}
\@namedef{wv@fam_clip_photographer_attributable@hi}{16.1}
\@namedef{wv@fam_clip_points_per_doubling@v}{$-$2.1}
\@namedef{wv@fam_clip_points_per_doubling@ci}{$-$2.4 to $-$1.8}
\@namedef{wv@fam_clip_points_per_doubling@lo}{$-$2.4}
\@namedef{wv@fam_clip_points_per_doubling@hi}{$-$1.8}
\@namedef{wv@fam_clip_reject_cosine_auroc@v}{0.806}
\@namedef{wv@fam_clip_reject_cosine_auroc@ci}{0.788 to 0.823}
\@namedef{wv@fam_clip_reject_cosine_auroc@lo}{0.788}
\@namedef{wv@fam_clip_reject_cosine_auroc@hi}{0.823}
\@namedef{wv@fam_clip_reject_margin_auroc@v}{0.852}
\@namedef{wv@fam_clip_reject_margin_auroc@ci}{0.834 to 0.869}
\@namedef{wv@fam_clip_reject_margin_auroc@lo}{0.834}
\@namedef{wv@fam_clip_reject_margin_auroc@hi}{0.869}
\@namedef{wv@fam_clip_reject_margin_false_acceptance_90@v}{59.1}
\@namedef{wv@fam_clip_top_1@v}{82.9}
\@namedef{wv@fam_clip_top_1@ci}{80.7 to 85.0}
\@namedef{wv@fam_clip_top_1@lo}{80.7}
\@namedef{wv@fam_clip_top_1@hi}{85.0}
\@namedef{wv@fam_clip_top_5@v}{90.7}
\@namedef{wv@fam_clip_unseen_r_at_10@v}{75.1}
\@namedef{wv@fam_clip_unseen_top_1@v}{54.1}
\@namedef{wv@fam_dino_cosine_false_acceptance_90@v}{35.0}
\@namedef{wv@fam_dino_geo_minus_random_pool_10@v}{$-$0.8}
\@namedef{wv@fam_dino_geo_minus_random_pool_10@ci}{$-$1.5 to $-$0.1}
\@namedef{wv@fam_dino_geo_minus_random_pool_10@lo}{$-$1.5}
\@namedef{wv@fam_dino_geo_minus_random_pool_10@hi}{$-$0.1}
\@namedef{wv@fam_dino_mrr@v}{0.936}
\@namedef{wv@fam_dino_photographer_attributable@v}{6.9}
\@namedef{wv@fam_dino_photographer_attributable@ci}{4.2 to 9.6}
\@namedef{wv@fam_dino_photographer_attributable@lo}{4.2}
\@namedef{wv@fam_dino_photographer_attributable@hi}{9.6}
\@namedef{wv@fam_dino_points_per_doubling@v}{$-$0.9}
\@namedef{wv@fam_dino_points_per_doubling@ci}{$-$1.1 to $-$0.8}
\@namedef{wv@fam_dino_points_per_doubling@lo}{$-$1.1}
\@namedef{wv@fam_dino_points_per_doubling@hi}{$-$0.8}
\@namedef{wv@fam_dino_reject_cosine_auroc@v}{0.915}
\@namedef{wv@fam_dino_reject_cosine_auroc@ci}{0.902 to 0.927}
\@namedef{wv@fam_dino_reject_cosine_auroc@lo}{0.902}
\@namedef{wv@fam_dino_reject_cosine_auroc@hi}{0.927}
\@namedef{wv@fam_dino_reject_margin_auroc@v}{0.946}
\@namedef{wv@fam_dino_reject_margin_auroc@ci}{0.936 to 0.956}
\@namedef{wv@fam_dino_reject_margin_auroc@lo}{0.936}
\@namedef{wv@fam_dino_reject_margin_auroc@hi}{0.956}
\@namedef{wv@fam_dino_reject_margin_false_acceptance_90@v}{11.9}
\@namedef{wv@fam_dino_top_1@v}{92.0}
\@namedef{wv@fam_dino_top_1@ci}{90.5 to 93.4}
\@namedef{wv@fam_dino_top_1@lo}{90.5}
\@namedef{wv@fam_dino_top_1@hi}{93.4}
\@namedef{wv@fam_dino_top_5@v}{95.3}
\@namedef{wv@fam_dino_unseen_r_at_10@v}{86.3}
\@namedef{wv@fam_dino_unseen_top_1@v}{74.4}
\@namedef{wv@fam_dinov2_cosine_false_acceptance_90@v}{38.3}
\@namedef{wv@fam_dinov2_geo_minus_random_pool_10@v}{$-$0.7}
\@namedef{wv@fam_dinov2_geo_minus_random_pool_10@ci}{$-$1.4 to $-$0.1}
\@namedef{wv@fam_dinov2_geo_minus_random_pool_10@lo}{$-$1.4}
\@namedef{wv@fam_dinov2_geo_minus_random_pool_10@hi}{$-$0.1}
\@namedef{wv@fam_dinov2_mrr@v}{0.943}
\@namedef{wv@fam_dinov2_photographer_attributable@v}{2.6}
\@namedef{wv@fam_dinov2_photographer_attributable@ci}{1.0 to 4.3}
\@namedef{wv@fam_dinov2_photographer_attributable@lo}{1.0}
\@namedef{wv@fam_dinov2_photographer_attributable@hi}{4.3}
\@namedef{wv@fam_dinov2_points_per_doubling@v}{$-$0.8}
\@namedef{wv@fam_dinov2_points_per_doubling@ci}{$-$1.0 to $-$0.6}
\@namedef{wv@fam_dinov2_points_per_doubling@lo}{$-$1.0}
\@namedef{wv@fam_dinov2_points_per_doubling@hi}{$-$0.6}
\@namedef{wv@fam_dinov2_reject_cosine_auroc@v}{0.896}
\@namedef{wv@fam_dinov2_reject_cosine_auroc@ci}{0.883 to 0.909}
\@namedef{wv@fam_dinov2_reject_cosine_auroc@lo}{0.883}
\@namedef{wv@fam_dinov2_reject_cosine_auroc@hi}{0.909}
\@namedef{wv@fam_dinov2_reject_margin_auroc@v}{0.927}
\@namedef{wv@fam_dinov2_reject_margin_auroc@ci}{0.914 to 0.940}
\@namedef{wv@fam_dinov2_reject_margin_auroc@lo}{0.914}
\@namedef{wv@fam_dinov2_reject_margin_auroc@hi}{0.940}
\@namedef{wv@fam_dinov2_reject_margin_false_acceptance_90@v}{19.6}
\@namedef{wv@fam_dinov2_top_1@v}{93.1}
\@namedef{wv@fam_dinov2_top_1@ci}{91.8 to 94.4}
\@namedef{wv@fam_dinov2_top_1@lo}{91.8}
\@namedef{wv@fam_dinov2_top_1@hi}{94.4}
\@namedef{wv@fam_dinov2_top_5@v}{95.7}
\@namedef{wv@fam_dinov2_unseen_r_at_10@v}{90.8}
\@namedef{wv@fam_dinov2_unseen_top_1@v}{81.8}
\@namedef{wv@fam_dinov3_cosine_false_acceptance_90@v}{21.6}
\@namedef{wv@fam_dinov3_geo_minus_random_pool_10@v}{$-$1.1}
\@namedef{wv@fam_dinov3_geo_minus_random_pool_10@ci}{$-$1.9 to $-$0.4}
\@namedef{wv@fam_dinov3_geo_minus_random_pool_10@lo}{$-$1.9}
\@namedef{wv@fam_dinov3_geo_minus_random_pool_10@hi}{$-$0.4}
\@namedef{wv@fam_dinov3_mrr@v}{0.956}
\@namedef{wv@fam_dinov3_photographer_attributable@v}{1.7}
\@namedef{wv@fam_dinov3_photographer_attributable@ci}{$-$0.3 to 3.7}
\@namedef{wv@fam_dinov3_photographer_attributable@lo}{$-$0.3}
\@namedef{wv@fam_dinov3_photographer_attributable@hi}{3.7}
\@namedef{wv@fam_dinov3_points_per_doubling@v}{$-$0.7}
\@namedef{wv@fam_dinov3_points_per_doubling@ci}{$-$0.8 to $-$0.5}
\@namedef{wv@fam_dinov3_points_per_doubling@lo}{$-$0.8}
\@namedef{wv@fam_dinov3_points_per_doubling@hi}{$-$0.5}
\@namedef{wv@fam_dinov3_reject_cosine_auroc@v}{0.926}
\@namedef{wv@fam_dinov3_reject_cosine_auroc@ci}{0.914 to 0.937}
\@namedef{wv@fam_dinov3_reject_cosine_auroc@lo}{0.914}
\@namedef{wv@fam_dinov3_reject_cosine_auroc@hi}{0.937}
\@namedef{wv@fam_dinov3_reject_margin_auroc@v}{0.959}
\@namedef{wv@fam_dinov3_reject_margin_auroc@ci}{0.949 to 0.967}
\@namedef{wv@fam_dinov3_reject_margin_auroc@lo}{0.949}
\@namedef{wv@fam_dinov3_reject_margin_auroc@hi}{0.967}
\@namedef{wv@fam_dinov3_reject_margin_false_acceptance_90@v}{7.7}
\@namedef{wv@fam_dinov3_top_1@v}{94.4}
\@namedef{wv@fam_dinov3_top_1@ci}{93.1 to 95.6}
\@namedef{wv@fam_dinov3_top_1@lo}{93.1}
\@namedef{wv@fam_dinov3_top_1@hi}{95.6}
\@namedef{wv@fam_dinov3_top_5@v}{96.9}
\@namedef{wv@fam_dinov3_unseen_r_at_10@v}{92.8}
\@namedef{wv@fam_dinov3_unseen_top_1@v}{85.2}
\@namedef{wv@fam_eva02-mim_cosine_false_acceptance_90@v}{63.2}
\@namedef{wv@fam_eva02-mim_geo_minus_random_pool_10@v}{$-$1.9}
\@namedef{wv@fam_eva02-mim_geo_minus_random_pool_10@ci}{$-$2.8 to $-$1.1}
\@namedef{wv@fam_eva02-mim_geo_minus_random_pool_10@lo}{$-$2.8}
\@namedef{wv@fam_eva02-mim_geo_minus_random_pool_10@hi}{$-$1.1}
\@namedef{wv@fam_eva02-mim_mrr@v}{0.880}
\@namedef{wv@fam_eva02-mim_photographer_attributable@v}{8.6}
\@namedef{wv@fam_eva02-mim_photographer_attributable@ci}{6.0 to 11.3}
\@namedef{wv@fam_eva02-mim_photographer_attributable@lo}{6.0}
\@namedef{wv@fam_eva02-mim_photographer_attributable@hi}{11.3}
\@namedef{wv@fam_eva02-mim_points_per_doubling@v}{$-$1.9}
\@namedef{wv@fam_eva02-mim_points_per_doubling@ci}{$-$2.2 to $-$1.7}
\@namedef{wv@fam_eva02-mim_points_per_doubling@lo}{$-$2.2}
\@namedef{wv@fam_eva02-mim_points_per_doubling@hi}{$-$1.7}
\@namedef{wv@fam_eva02-mim_reject_cosine_auroc@v}{0.828}
\@namedef{wv@fam_eva02-mim_reject_cosine_auroc@ci}{0.813 to 0.845}
\@namedef{wv@fam_eva02-mim_reject_cosine_auroc@lo}{0.813}
\@namedef{wv@fam_eva02-mim_reject_cosine_auroc@hi}{0.845}
\@namedef{wv@fam_eva02-mim_reject_margin_auroc@v}{0.864}
\@namedef{wv@fam_eva02-mim_reject_margin_auroc@ci}{0.847 to 0.879}
\@namedef{wv@fam_eva02-mim_reject_margin_auroc@lo}{0.847}
\@namedef{wv@fam_eva02-mim_reject_margin_auroc@hi}{0.879}
\@namedef{wv@fam_eva02-mim_reject_margin_false_acceptance_90@v}{50.4}
\@namedef{wv@fam_eva02-mim_top_1@v}{84.5}
\@namedef{wv@fam_eva02-mim_top_1@ci}{82.5 to 86.3}
\@namedef{wv@fam_eva02-mim_top_1@lo}{82.5}
\@namedef{wv@fam_eva02-mim_top_1@hi}{86.3}
\@namedef{wv@fam_eva02-mim_top_5@v}{92.1}
\@namedef{wv@fam_eva02-mim_unseen_r_at_10@v}{80.4}
\@namedef{wv@fam_eva02-mim_unseen_top_1@v}{63.2}
\@namedef{wv@fam_ijepa_cosine_false_acceptance_90@v}{79.5}
\@namedef{wv@fam_ijepa_geo_minus_random_pool_10@v}{$-$4.5}
\@namedef{wv@fam_ijepa_geo_minus_random_pool_10@ci}{$-$6.3 to $-$2.8}
\@namedef{wv@fam_ijepa_geo_minus_random_pool_10@lo}{$-$6.3}
\@namedef{wv@fam_ijepa_geo_minus_random_pool_10@hi}{$-$2.8}
\@namedef{wv@fam_ijepa_mrr@v}{0.652}
\@namedef{wv@fam_ijepa_photographer_attributable@v}{10.1}
\@namedef{wv@fam_ijepa_photographer_attributable@ci}{7.4 to 12.9}
\@namedef{wv@fam_ijepa_photographer_attributable@lo}{7.4}
\@namedef{wv@fam_ijepa_photographer_attributable@hi}{12.9}
\@namedef{wv@fam_ijepa_points_per_doubling@v}{$-$5.6}
\@namedef{wv@fam_ijepa_points_per_doubling@ci}{$-$6.1 to $-$5.1}
\@namedef{wv@fam_ijepa_points_per_doubling@lo}{$-$6.1}
\@namedef{wv@fam_ijepa_points_per_doubling@hi}{$-$5.1}
\@namedef{wv@fam_ijepa_reject_cosine_auroc@v}{0.698}
\@namedef{wv@fam_ijepa_reject_cosine_auroc@ci}{0.678 to 0.717}
\@namedef{wv@fam_ijepa_reject_cosine_auroc@lo}{0.678}
\@namedef{wv@fam_ijepa_reject_cosine_auroc@hi}{0.717}
\@namedef{wv@fam_ijepa_reject_margin_auroc@v}{0.677}
\@namedef{wv@fam_ijepa_reject_margin_auroc@ci}{0.655 to 0.700}
\@namedef{wv@fam_ijepa_reject_margin_auroc@lo}{0.655}
\@namedef{wv@fam_ijepa_reject_margin_auroc@hi}{0.700}
\@namedef{wv@fam_ijepa_reject_margin_false_acceptance_90@v}{82.9}
\@namedef{wv@fam_ijepa_top_1@v}{55.6}
\@namedef{wv@fam_ijepa_top_1@ci}{51.9 to 59.2}
\@namedef{wv@fam_ijepa_top_1@lo}{51.9}
\@namedef{wv@fam_ijepa_top_1@hi}{59.2}
\@namedef{wv@fam_ijepa_top_5@v}{76.8}
\@namedef{wv@fam_ijepa_unseen_r_at_10@v}{56.9}
\@namedef{wv@fam_ijepa_unseen_top_1@v}{34.2}
\@namedef{wv@fam_mae_cosine_false_acceptance_90@v}{84.8}
\@namedef{wv@fam_mae_geo_minus_random_pool_10@v}{$-$2.8}
\@namedef{wv@fam_mae_geo_minus_random_pool_10@ci}{$-$4.7 to $-$0.9}
\@namedef{wv@fam_mae_geo_minus_random_pool_10@lo}{$-$4.7}
\@namedef{wv@fam_mae_geo_minus_random_pool_10@hi}{$-$0.9}
\@namedef{wv@fam_mae_mrr@v}{0.546}
\@namedef{wv@fam_mae_photographer_attributable@v}{14.8}
\@namedef{wv@fam_mae_photographer_attributable@ci}{12.1 to 17.6}
\@namedef{wv@fam_mae_photographer_attributable@lo}{12.1}
\@namedef{wv@fam_mae_photographer_attributable@hi}{17.6}
\@namedef{wv@fam_mae_points_per_doubling@v}{$-$6.3}
\@namedef{wv@fam_mae_points_per_doubling@ci}{$-$6.7 to $-$5.9}
\@namedef{wv@fam_mae_points_per_doubling@lo}{$-$6.7}
\@namedef{wv@fam_mae_points_per_doubling@hi}{$-$5.9}
\@namedef{wv@fam_mae_reject_cosine_auroc@v}{0.619}
\@namedef{wv@fam_mae_reject_cosine_auroc@ci}{0.605 to 0.633}
\@namedef{wv@fam_mae_reject_cosine_auroc@lo}{0.605}
\@namedef{wv@fam_mae_reject_cosine_auroc@hi}{0.633}
\@namedef{wv@fam_mae_reject_margin_auroc@v}{0.616}
\@namedef{wv@fam_mae_reject_margin_auroc@ci}{0.599 to 0.634}
\@namedef{wv@fam_mae_reject_margin_auroc@lo}{0.599}
\@namedef{wv@fam_mae_reject_margin_auroc@hi}{0.634}
\@namedef{wv@fam_mae_reject_margin_false_acceptance_90@v}{86.5}
\@namedef{wv@fam_mae_top_1@v}{46.8}
\@namedef{wv@fam_mae_top_1@ci}{43.7 to 50.0}
\@namedef{wv@fam_mae_top_1@lo}{43.7}
\@namedef{wv@fam_mae_top_1@hi}{50.0}
\@namedef{wv@fam_mae_top_5@v}{63.5}
\@namedef{wv@fam_mae_unseen_r_at_10@v}{32.1}
\@namedef{wv@fam_mae_unseen_top_1@v}{14.3}
\@namedef{wv@fam_radio_cosine_false_acceptance_90@v}{25.5}
\@namedef{wv@fam_radio_geo_minus_random_pool_10@v}{$-$0.4}
\@namedef{wv@fam_radio_geo_minus_random_pool_10@ci}{$-$0.8 to 0.0}
\@namedef{wv@fam_radio_geo_minus_random_pool_10@lo}{$-$0.8}
\@namedef{wv@fam_radio_geo_minus_random_pool_10@hi}{0.0}
\@namedef{wv@fam_radio_mrr@v}{0.956}
\@namedef{wv@fam_radio_photographer_attributable@v}{3.3}
\@namedef{wv@fam_radio_photographer_attributable@ci}{1.6 to 5.0}
\@namedef{wv@fam_radio_photographer_attributable@lo}{1.6}
\@namedef{wv@fam_radio_photographer_attributable@hi}{5.0}
\@namedef{wv@fam_radio_points_per_doubling@v}{$-$0.6}
\@namedef{wv@fam_radio_points_per_doubling@ci}{$-$0.8 to $-$0.5}
\@namedef{wv@fam_radio_points_per_doubling@lo}{$-$0.8}
\@namedef{wv@fam_radio_points_per_doubling@hi}{$-$0.5}
\@namedef{wv@fam_radio_reject_cosine_auroc@v}{0.920}
\@namedef{wv@fam_radio_reject_cosine_auroc@ci}{0.909 to 0.931}
\@namedef{wv@fam_radio_reject_cosine_auroc@lo}{0.909}
\@namedef{wv@fam_radio_reject_cosine_auroc@hi}{0.931}
\@namedef{wv@fam_radio_reject_margin_auroc@v}{0.947}
\@namedef{wv@fam_radio_reject_margin_auroc@ci}{0.935 to 0.958}
\@namedef{wv@fam_radio_reject_margin_auroc@lo}{0.935}
\@namedef{wv@fam_radio_reject_margin_auroc@hi}{0.958}
\@namedef{wv@fam_radio_reject_margin_false_acceptance_90@v}{12.2}
\@namedef{wv@fam_radio_top_1@v}{94.7}
\@namedef{wv@fam_radio_top_1@ci}{93.5 to 95.8}
\@namedef{wv@fam_radio_top_1@lo}{93.5}
\@namedef{wv@fam_radio_top_1@hi}{95.8}
\@namedef{wv@fam_radio_top_5@v}{96.5}
\@namedef{wv@fam_radio_unseen_r_at_10@v}{91.8}
\@namedef{wv@fam_radio_unseen_top_1@v}{84.3}
\@namedef{wv@fam_siglip2_cosine_false_acceptance_90@v}{43.8}
\@namedef{wv@fam_siglip2_geo_minus_random_pool_10@v}{$-$1.0}
\@namedef{wv@fam_siglip2_geo_minus_random_pool_10@ci}{$-$1.7 to $-$0.3}
\@namedef{wv@fam_siglip2_geo_minus_random_pool_10@lo}{$-$1.7}
\@namedef{wv@fam_siglip2_geo_minus_random_pool_10@hi}{$-$0.3}
\@namedef{wv@fam_siglip2_mrr@v}{0.929}
\@namedef{wv@fam_siglip2_photographer_attributable@v}{6.2}
\@namedef{wv@fam_siglip2_photographer_attributable@ci}{3.9 to 8.7}
\@namedef{wv@fam_siglip2_photographer_attributable@lo}{3.9}
\@namedef{wv@fam_siglip2_photographer_attributable@hi}{8.7}
\@namedef{wv@fam_siglip2_points_per_doubling@v}{$-$1.0}
\@namedef{wv@fam_siglip2_points_per_doubling@ci}{$-$1.2 to $-$0.8}
\@namedef{wv@fam_siglip2_points_per_doubling@lo}{$-$1.2}
\@namedef{wv@fam_siglip2_points_per_doubling@hi}{$-$0.8}
\@namedef{wv@fam_siglip2_reject_cosine_auroc@v}{0.877}
\@namedef{wv@fam_siglip2_reject_cosine_auroc@ci}{0.861 to 0.892}
\@namedef{wv@fam_siglip2_reject_cosine_auroc@lo}{0.861}
\@namedef{wv@fam_siglip2_reject_cosine_auroc@hi}{0.892}
\@namedef{wv@fam_siglip2_reject_margin_auroc@v}{0.916}
\@namedef{wv@fam_siglip2_reject_margin_auroc@ci}{0.902 to 0.929}
\@namedef{wv@fam_siglip2_reject_margin_auroc@lo}{0.902}
\@namedef{wv@fam_siglip2_reject_margin_auroc@hi}{0.929}
\@namedef{wv@fam_siglip2_reject_margin_false_acceptance_90@v}{27.7}
\@namedef{wv@fam_siglip2_top_1@v}{91.2}
\@namedef{wv@fam_siglip2_top_1@ci}{89.6 to 92.6}
\@namedef{wv@fam_siglip2_top_1@lo}{89.6}
\@namedef{wv@fam_siglip2_top_1@hi}{92.6}
\@namedef{wv@fam_siglip2_top_5@v}{94.7}
\@namedef{wv@fam_siglip2_unseen_r_at_10@v}{86.7}
\@namedef{wv@fam_siglip2_unseen_top_1@v}{75.0}
\@namedef{wv@fam_vit-supervised_cosine_false_acceptance_90@v}{52.7}
\@namedef{wv@fam_vit-supervised_geo_minus_random_pool_10@v}{$-$1.7}
\@namedef{wv@fam_vit-supervised_geo_minus_random_pool_10@ci}{$-$2.6 to $-$0.8}
\@namedef{wv@fam_vit-supervised_geo_minus_random_pool_10@lo}{$-$2.6}
\@namedef{wv@fam_vit-supervised_geo_minus_random_pool_10@hi}{$-$0.8}
\@namedef{wv@fam_vit-supervised_mrr@v}{0.914}
\@namedef{wv@fam_vit-supervised_photographer_attributable@v}{11.7}
\@namedef{wv@fam_vit-supervised_photographer_attributable@ci}{8.7 to 14.8}
\@namedef{wv@fam_vit-supervised_photographer_attributable@lo}{8.7}
\@namedef{wv@fam_vit-supervised_photographer_attributable@hi}{14.8}
\@namedef{wv@fam_vit-supervised_points_per_doubling@v}{$-$1.3}
\@namedef{wv@fam_vit-supervised_points_per_doubling@ci}{$-$1.5 to $-$1.1}
\@namedef{wv@fam_vit-supervised_points_per_doubling@lo}{$-$1.5}
\@namedef{wv@fam_vit-supervised_points_per_doubling@hi}{$-$1.1}
\@namedef{wv@fam_vit-supervised_reject_cosine_auroc@v}{0.865}
\@namedef{wv@fam_vit-supervised_reject_cosine_auroc@ci}{0.850 to 0.880}
\@namedef{wv@fam_vit-supervised_reject_cosine_auroc@lo}{0.850}
\@namedef{wv@fam_vit-supervised_reject_cosine_auroc@hi}{0.880}
\@namedef{wv@fam_vit-supervised_reject_margin_auroc@v}{0.917}
\@namedef{wv@fam_vit-supervised_reject_margin_auroc@ci}{0.905 to 0.930}
\@namedef{wv@fam_vit-supervised_reject_margin_auroc@lo}{0.905}
\@namedef{wv@fam_vit-supervised_reject_margin_auroc@hi}{0.930}
\@namedef{wv@fam_vit-supervised_reject_margin_false_acceptance_90@v}{31.2}
\@namedef{wv@fam_vit-supervised_top_1@v}{89.4}
\@namedef{wv@fam_vit-supervised_top_1@ci}{87.5 to 91.1}
\@namedef{wv@fam_vit-supervised_top_1@lo}{87.5}
\@namedef{wv@fam_vit-supervised_top_1@hi}{91.1}
\@namedef{wv@fam_vit-supervised_top_5@v}{93.7}
\@namedef{wv@fam_vit-supervised_unseen_r_at_10@v}{78.6}
\@namedef{wv@fam_vit-supervised_unseen_top_1@v}{62.5}
\makeatother


==> generated/numbers.tex <==
\makeatletter
\newcommand{\wv}[1]{\@ifundefined{wv@#1@v}{\textbf{\color{red}MISSING:\detokenize{#1}}}{\csname wv@#1@v\endcsname}}
\newcommand{\wvci}[1]{\@ifundefined{wv@#1@ci}{\textbf{\color{red}MISSING:\detokenize{#1}}}{\csname wv@#1@ci\endcsname}}
\newcommand{\wvlo}[1]{\@ifundefined{wv@#1@lo}{\textbf{\color{red}MISSING:\detokenize{#1}}}{\csname wv@#1@lo\endcsname}}
\newcommand{\wvhi}[1]{\@ifundefined{wv@#1@hi}{\textbf{\color{red}MISSING:\detokenize{#1}}}{\csname wv@#1@hi\endcsname}}
\@namedef{wv@clip_families_count@v}{34}
\@namedef{wv@clip_families_error_share@v}{12.5}
\@namedef{wv@clip_families_error_share@ci}{7.7 to 17.8}
\@namedef{wv@clip_families_error_share@lo}{7.7}
\@namedef{wv@clip_families_error_share@hi}{17.8}
\@namedef{wv@clip_families_errors@v}{289}
\@namedef{wv@clip_families_inside_error_rate@v}{17.9}
\@namedef{wv@clip_families_inside_error_rate@ci}{14.2 to 21.9}
\@namedef{wv@clip_families_inside_error_rate@lo}{14.2}
\@namedef{wv@clip_families_inside_error_rate@hi}{21.9}
\@namedef{wv@clip_families_outside_error_rate@v}{16.7}
\@namedef{wv@clip_families_outside_error_rate@ci}{14.2 to 19.3}
\@namedef{wv@clip_families_outside_error_rate@lo}{14.2}
\@namedef{wv@clip_families_outside_error_rate@hi}{19.3}
\@namedef{wv@clip_families_statue_share@v}{34.0}
\@namedef{wv@clip_families_statues@v}{104}
\@namedef{wv@clip_geo_minus_random_pool_10@v}{$-$2.1}
\@namedef{wv@clip_geo_minus_random_pool_10@ci}{$-$3.1 to $-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_10@lo}{$-$3.1}
\@namedef{wv@clip_geo_minus_random_pool_10@hi}{$-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_100@v}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_100@ci}{$-$2.6 to $-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_100@lo}{$-$2.6}
\@namedef{wv@clip_geo_minus_random_pool_100@hi}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_150@v}{$-$1.6}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_150@ci}{$-$2.3 to $-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_150@lo}{$-$2.3}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_150@hi}{$-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_50@v}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_50@ci}{$-$2.5 to $-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_50@lo}{$-$2.5}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_50@hi}{$-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_9@v}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_9@ci}{$-$2.6 to $-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_9@lo}{$-$2.6}
\@namedef{wv@clip_geo_minus_random_pool_100_noise_9@hi}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_150@v}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_150@ci}{$-$2.2 to $-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_150@lo}{$-$2.2}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_150@hi}{$-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_50@v}{$-$1.9}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_50@ci}{$-$2.7 to $-$1.1}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_50@lo}{$-$2.7}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_50@hi}{$-$1.1}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_9@v}{$-$2.1}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_9@ci}{$-$2.9 to $-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_9@lo}{$-$2.9}
\@namedef{wv@clip_geo_minus_random_pool_10_noise_9@hi}{$-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_15@v}{$-$1.7}
\@namedef{wv@clip_geo_minus_random_pool_15@ci}{$-$2.7 to $-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_15@lo}{$-$2.7}
\@namedef{wv@clip_geo_minus_random_pool_15@hi}{$-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_150@v}{$-$1.1}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_150@ci}{$-$1.8 to $-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_150@lo}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_150@hi}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_50@v}{$-$1.7}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_50@ci}{$-$2.7 to $-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_50@lo}{$-$2.7}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_50@hi}{$-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_9@v}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_9@ci}{$-$2.7 to $-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_9@lo}{$-$2.7}
\@namedef{wv@clip_geo_minus_random_pool_15_noise_9@hi}{$-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_2@v}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_2@ci}{$-$1.8 to $-$0.3}
\@namedef{wv@clip_geo_minus_random_pool_2@lo}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_2@hi}{$-$0.3}
\@namedef{wv@clip_geo_minus_random_pool_20@v}{$-$1.7}
\@namedef{wv@clip_geo_minus_random_pool_20@ci}{$-$2.6 to $-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_20@lo}{$-$2.6}
\@namedef{wv@clip_geo_minus_random_pool_20@hi}{$-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_200@v}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_200@ci}{$-$1.5 to $-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_200@lo}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_200@hi}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_150@v}{$-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_150@ci}{$-$1.4 to $-$0.3}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_150@lo}{$-$1.4}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_150@hi}{$-$0.3}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_50@v}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_50@ci}{$-$1.5 to $-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_50@lo}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_50@hi}{$-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_9@v}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_9@ci}{$-$1.5 to $-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_9@lo}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_200_noise_9@hi}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_150@v}{$-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_150@ci}{$-$2.0 to $-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_150@lo}{$-$2.0}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_150@hi}{$-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_50@v}{$-$1.6}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_50@ci}{$-$2.4 to $-$0.7}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_50@lo}{$-$2.4}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_50@hi}{$-$0.7}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_9@v}{$-$1.6}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_9@ci}{$-$2.5 to $-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_9@lo}{$-$2.5}
\@namedef{wv@clip_geo_minus_random_pool_20_noise_9@hi}{$-$0.8}
\@namedef{wv@clip_geo_minus_random_pool_294@v}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294@ci}{0.0 to 0.0}
\@namedef{wv@clip_geo_minus_random_pool_294@lo}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294@hi}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_150@v}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_150@ci}{0.0 to 0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_150@lo}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_150@hi}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_50@v}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_50@ci}{0.0 to 0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_50@lo}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_50@hi}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_9@v}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_9@ci}{0.0 to 0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_9@lo}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_294_noise_9@hi}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_150@v}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_150@ci}{$-$0.9 to 0.0}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_150@lo}{$-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_150@hi}{0.0}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_50@v}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_50@ci}{$-$1.5 to $-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_50@lo}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_50@hi}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_9@v}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_9@ci}{$-$1.6 to $-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_9@lo}{$-$1.6}
\@namedef{wv@clip_geo_minus_random_pool_2_noise_9@hi}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_3@v}{$-$1.1}
\@namedef{wv@clip_geo_minus_random_pool_3@ci}{$-$2.0 to $-$0.3}
\@namedef{wv@clip_geo_minus_random_pool_3@lo}{$-$2.0}
\@namedef{wv@clip_geo_minus_random_pool_3@hi}{$-$0.3}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_150@v}{$-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_150@ci}{$-$1.0 to $-$0.1}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_150@lo}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_150@hi}{$-$0.1}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_50@v}{$-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_50@ci}{$-$1.5 to $-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_50@lo}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_50@hi}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_9@v}{$-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_9@ci}{$-$2.0 to $-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_9@lo}{$-$2.0}
\@namedef{wv@clip_geo_minus_random_pool_3_noise_9@hi}{$-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_5@v}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_5@ci}{$-$2.7 to $-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_5@lo}{$-$2.7}
\@namedef{wv@clip_geo_minus_random_pool_5@hi}{$-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_50@v}{$-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_50@ci}{$-$2.1 to $-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_50@lo}{$-$2.1}
\@namedef{wv@clip_geo_minus_random_pool_50@hi}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_150@v}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_150@ci}{$-$2.6 to $-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_150@lo}{$-$2.6}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_150@hi}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_50@v}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_50@ci}{$-$2.3 to $-$0.7}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_50@lo}{$-$2.3}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_50@hi}{$-$0.7}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_9@v}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_9@ci}{$-$2.4 to $-$0.6}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_9@lo}{$-$2.4}
\@namedef{wv@clip_geo_minus_random_pool_50_noise_9@hi}{$-$0.6}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_150@v}{$-$0.9}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_150@ci}{$-$1.5 to $-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_150@lo}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_150@hi}{$-$0.4}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_50@v}{$-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_50@ci}{$-$1.9 to $-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_50@lo}{$-$1.9}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_50@hi}{$-$0.5}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_9@v}{$-$1.5}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_9@ci}{$-$2.4 to $-$0.7}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_9@lo}{$-$2.4}
\@namedef{wv@clip_geo_minus_random_pool_5_noise_9@hi}{$-$0.7}
\@namedef{wv@clip_geo_minus_random_pool_8@v}{$-$1.8}
\@namedef{wv@clip_geo_minus_random_pool_8@ci}{$-$2.8 to $-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_8@lo}{$-$2.8}
\@namedef{wv@clip_geo_minus_random_pool_8@hi}{$-$1.0}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_150@v}{$-$1.2}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_150@ci}{$-$1.9 to $-$0.6}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_150@lo}{$-$1.9}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_150@hi}{$-$0.6}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_50@v}{$-$1.9}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_50@ci}{$-$2.6 to $-$1.1}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_50@lo}{$-$2.6}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_50@hi}{$-$1.1}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_9@v}{$-$1.9}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_9@ci}{$-$2.8 to $-$1.1}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_9@lo}{$-$2.8}
\@namedef{wv@clip_geo_minus_random_pool_8_noise_9@hi}{$-$1.1}
\@namedef{wv@clip_geo_permutation_mean_null@v}{0.0}
\@namedef{wv@clip_geo_permutation_mean_null@ci}{$-$0.5 to 0.6}
\@namedef{wv@clip_geo_permutation_mean_null@lo}{$-$0.5}
\@namedef{wv@clip_geo_permutation_mean_null@hi}{0.6}
\@namedef{wv@clip_geo_permutation_mean_observed@v}{$-$1.9}
\@namedef{wv@clip_geo_permutation_mean_p_value@v}{0.005}
\@namedef{wv@clip_geo_permutation_permutations@v}{200}
\@namedef{wv@clip_geo_permutation_pool_10_null_mean@v}{$-$0.1}
\@namedef{wv@clip_geo_permutation_pool_10_null_mean@ci}{$-$0.7 to 0.6}
\@namedef{wv@clip_geo_permutation_pool_10_null_mean@lo}{$-$0.7}
\@namedef{wv@clip_geo_permutation_pool_10_null_mean@hi}{0.6}
\@namedef{wv@clip_geo_permutation_pool_10_p_value@v}{0.005}
\@namedef{wv@clip_geo_permutation_pool_20_null_mean@v}{0.2}
\@namedef{wv@clip_geo_permutation_pool_20_null_mean@ci}{$-$0.5 to 0.9}
\@namedef{wv@clip_geo_permutation_pool_20_null_mean@lo}{$-$0.5}
\@namedef{wv@clip_geo_permutation_pool_20_null_mean@hi}{0.9}
\@namedef{wv@clip_geo_permutation_pool_20_p_value@v}{0.005}
\@namedef{wv@clip_geo_permutation_pool_5_null_mean@v}{0.0}
\@namedef{wv@clip_geo_permutation_pool_5_null_mean@ci}{$-$0.6 to 0.6}
\@namedef{wv@clip_geo_permutation_pool_5_null_mean@lo}{$-$0.6}
\@namedef{wv@clip_geo_permutation_pool_5_null_mean@hi}{0.6}
\@namedef{wv@clip_geo_permutation_pool_5_p_value@v}{0.005}
\@namedef{wv@clip_groups_changed_queries@v}{5}
\@namedef{wv@clip_groups_merged_gain@v}{0.3}
\@namedef{wv@clip_groups_merged_gain@ci}{0.0 to 0.7}
\@namedef{wv@clip_groups_merged_gain@lo}{0.0}
\@namedef{wv@clip_groups_merged_gain@hi}{0.7}
\@namedef{wv@clip_groups_merged_top_1@v}{83.2}
\@namedef{wv@clip_groups_merged_top_1@ci}{81.0 to 85.3}
\@namedef{wv@clip_groups_merged_top_1@lo}{81.0}
\@namedef{wv@clip_groups_merged_top_1@hi}{85.3}
\@namedef{wv@clip_minus_dinov3_top_1@v}{$-$11.5}
\@namedef{wv@clip_minus_dinov3_top_1@ci}{$-$13.5 to $-$9.6}
\@namedef{wv@clip_minus_dinov3_top_1@lo}{$-$13.5}
\@namedef{wv@clip_minus_dinov3_top_1@hi}{$-$9.6}
\@namedef{wv@clip_minus_siglip2_top_1@v}{$-$8.3}
\@namedef{wv@clip_minus_siglip2_top_1@ci}{$-$10.1 to $-$6.5}
\@namedef{wv@clip_minus_siglip2_top_1@lo}{$-$10.1}
\@namedef{wv@clip_minus_siglip2_top_1@hi}{$-$6.5}
\@namedef{wv@clip_photographer_attributable@v}{13.2}
\@namedef{wv@clip_photographer_attributable@ci}{10.5 to 16.1}
\@namedef{wv@clip_photographer_attributable@lo}{10.5}
\@namedef{wv@clip_photographer_attributable@hi}{16.1}
\@namedef{wv@clip_photographer_raw_gap@v}{27.9}
\@namedef{wv@clip_photographer_raw_gap@ci}{23.7 to 32.4}
\@namedef{wv@clip_photographer_raw_gap@lo}{23.7}
\@namedef{wv@clip_photographer_raw_gap@hi}{32.4}
\@namedef{wv@clip_photographer_reference_cost@v}{14.7}
\@namedef{wv@clip_photographer_reference_cost@ci}{11.8 to 17.8}
\@namedef{wv@clip_photographer_reference_cost@lo}{11.8}
\@namedef{wv@clip_photographer_reference_cost@hi}{17.8}
\@namedef{wv@clip_points_per_doubling@v}{$-$2.1}
\@namedef{wv@clip_points_per_doubling@ci}{$-$2.4 to $-$1.8}
\@namedef{wv@clip_points_per_doubling@lo}{$-$2.4}
\@namedef{wv@clip_points_per_doubling@hi}{$-$1.8}
\@namedef{wv@clip_reject_cosine_auroc@v}{0.806}
\@namedef{wv@clip_reject_cosine_auroc@ci}{0.788 to 0.823}
\@namedef{wv@clip_reject_cosine_auroc@lo}{0.788}
\@namedef{wv@clip_reject_cosine_auroc@hi}{0.823}
\@namedef{wv@clip_reject_cosine_false_acceptance_90@v}{67.4}
\@namedef{wv@clip_reject_cosine_known_acceptance_90@v}{90.0}
\@namedef{wv@clip_reject_knn_auroc@v}{0.571}
\@namedef{wv@clip_reject_knn_auroc@ci}{0.559 to 0.585}
\@namedef{wv@clip_reject_knn_auroc@lo}{0.559}
\@namedef{wv@clip_reject_knn_auroc@hi}{0.585}
\@namedef{wv@clip_reject_knn_false_acceptance_90@v}{87.0}
\@namedef{wv@clip_reject_knn_known_acceptance_90@v}{89.9}
\@namedef{wv@clip_reject_knn_minus_cosine_auroc@v}{$-$0.235}
\@namedef{wv@clip_reject_knn_minus_cosine_auroc@ci}{$-$0.250 to $-$0.221}
\@namedef{wv@clip_reject_knn_minus_cosine_auroc@lo}{$-$0.250}
\@namedef{wv@clip_reject_knn_minus_cosine_auroc@hi}{$-$0.221}
\@namedef{wv@clip_reject_margin_auroc@v}{0.852}
\@namedef{wv@clip_reject_margin_auroc@ci}{0.834 to 0.869}
\@namedef{wv@clip_reject_margin_auroc@lo}{0.834}
\@namedef{wv@clip_reject_margin_auroc@hi}{0.869}
\@namedef{wv@clip_reject_margin_false_acceptance_90@v}{59.1}
\@namedef{wv@clip_reject_margin_known_acceptance_90@v}{89.9}
\@namedef{wv@clip_reject_margin_minus_cosine_auroc@v}{0.046}
\@namedef{wv@clip_reject_margin_minus_cosine_auroc@ci}{0.031 to 0.060}
\@namedef{wv@clip_reject_margin_minus_cosine_auroc@lo}{0.031}
\@namedef{wv@clip_reject_margin_minus_cosine_auroc@hi}{0.060}
\@namedef{wv@clip_soft_prior_gps10_fold_0_weight@v}{1}
\@namedef{wv@clip_soft_prior_gps10_fold_1_weight@v}{1}
\@namedef{wv@clip_soft_prior_gps10_fold_2_weight@v}{1}
\@namedef{wv@clip_soft_prior_gps10_fold_3_weight@v}{1}
\@namedef{wv@clip_soft_prior_gps10_fold_4_weight@v}{1}
\@namedef{wv@clip_soft_prior_gps10_gain@v}{15.2}
\@namedef{wv@clip_soft_prior_gps10_gain@ci}{13.2 to 17.4}
\@namedef{wv@clip_soft_prior_gps10_gain@lo}{13.2}
\@namedef{wv@clip_soft_prior_gps10_gain@hi}{17.4}
\@namedef{wv@clip_soft_prior_gps10_location_only_top_1@v}{90.6}
\@namedef{wv@clip_soft_prior_gps10_location_only_top_1@ci}{87.5 to 93.2}
\@namedef{wv@clip_soft_prior_gps10_location_only_top_1@lo}{87.5}
\@namedef{wv@clip_soft_prior_gps10_location_only_top_1@hi}{93.2}
\@namedef{wv@clip_soft_prior_gps10_top_1@v}{98.0}
\@namedef{wv@clip_soft_prior_gps10_top_1@ci}{97.2 to 98.7}
\@namedef{wv@clip_soft_prior_gps10_top_1@lo}{97.2}
\@namedef{wv@clip_soft_prior_gps10_top_1@hi}{98.7}
\@namedef{wv@clip_soft_prior_gps10_w0.005_top_1@v}{85.1}
\@namedef{wv@clip_soft_prior_gps10_w0.01_top_1@v}{86.6}
\@namedef{wv@clip_soft_prior_gps10_w0.02_top_1@v}{88.5}
\@namedef{wv@clip_soft_prior_gps10_w0.05_top_1@v}{92.2}
\@namedef{wv@clip_soft_prior_gps10_w0.1_top_1@v}{94.8}
\@namedef{wv@clip_soft_prior_gps10_w0.2_top_1@v}{96.7}
\@namedef{wv@clip_soft_prior_gps10_w0.5_top_1@v}{97.9}
\@namedef{wv@clip_soft_prior_gps10_w0_top_1@v}{82.8}
\@namedef{wv@clip_soft_prior_gps10_w10_top_1@v}{93.5}
\@namedef{wv@clip_soft_prior_gps10_w1_top_1@v}{98.0}
\@namedef{wv@clip_soft_prior_gps10_w20_top_1@v}{92.3}
\@namedef{wv@clip_soft_prior_gps10_w2_top_1@v}{97.4}
\@namedef{wv@clip_soft_prior_gps10_w5_top_1@v}{95.5}
\@namedef{wv@clip_soft_prior_gps25_fold_0_weight@v}{0.5}
\@namedef{wv@clip_soft_prior_gps25_fold_1_weight@v}{0.5}
\@namedef{wv@clip_soft_prior_gps25_fold_2_weight@v}{0.5}
\@namedef{wv@clip_soft_prior_gps25_fold_3_weight@v}{0.5}
\@namedef{wv@clip_soft_prior_gps25_fold_4_weight@v}{0.5}
\@namedef{wv@clip_soft_prior_gps25_gain@v}{13.8}
\@namedef{wv@clip_soft_prior_gps25_gain@ci}{11.9 to 15.9}
\@namedef{wv@clip_soft_prior_gps25_gain@lo}{11.9}
\@namedef{wv@clip_soft_prior_gps25_gain@hi}{15.9}
\@namedef{wv@clip_soft_prior_gps25_location_only_top_1@v}{74.8}
\@namedef{wv@clip_soft_prior_gps25_location_only_top_1@ci}{70.2 to 79.3}
\@namedef{wv@clip_soft_prior_gps25_location_only_top_1@lo}{70.2}
\@namedef{wv@clip_soft_prior_gps25_location_only_top_1@hi}{79.3}
\@namedef{wv@clip_soft_prior_gps25_top_1@v}{96.7}
\@namedef{wv@clip_soft_prior_gps25_top_1@ci}{95.7 to 97.6}
\@namedef{wv@clip_soft_prior_gps25_top_1@lo}{95.7}
\@namedef{wv@clip_soft_prior_gps25_top_1@hi}{97.6}
\@namedef{wv@clip_soft_prior_gps25_w0.005_top_1@v}{84.7}
\@namedef{wv@clip_soft_prior_gps25_w0.01_top_1@v}{86.4}
\@namedef{wv@clip_soft_prior_gps25_w0.02_top_1@v}{88.3}
\@namedef{wv@clip_soft_prior_gps25_w0.05_top_1@v}{91.9}
\@namedef{wv@clip_soft_prior_gps25_w0.1_top_1@v}{94.3}
\@namedef{wv@clip_soft_prior_gps25_w0.2_top_1@v}{96.0}
\@namedef{wv@clip_soft_prior_gps25_w0.5_top_1@v}{96.7}
\@namedef{wv@clip_soft_prior_gps25_w0_top_1@v}{82.8}
\@namedef{wv@clip_soft_prior_gps25_w10_top_1@v}{78.0}
\@namedef{wv@clip_soft_prior_gps25_w1_top_1@v}{95.1}
\@namedef{wv@clip_soft_prior_gps25_w20_top_1@v}{76.6}
\@namedef{wv@clip_soft_prior_gps25_w2_top_1@v}{89.4}
\@namedef{wv@clip_soft_prior_gps25_w5_top_1@v}{81.2}
\@namedef{wv@clip_soft_prior_gps50_fold_0_weight@v}{0.2}
\@namedef{wv@clip_soft_prior_gps50_fold_1_weight@v}{0.2}
\@namedef{wv@clip_soft_prior_gps50_fold_2_weight@v}{0.2}
\@namedef{wv@clip_soft_prior_gps50_fold_3_weight@v}{0.2}
\@namedef{wv@clip_soft_prior_gps50_fold_4_weight@v}{0.2}
\@namedef{wv@clip_soft_prior_gps50_gain@v}{11.6}
\@namedef{wv@clip_soft_prior_gps50_gain@ci}{9.8 to 13.6}
\@namedef{wv@clip_soft_prior_gps50_gain@lo}{9.8}
\@namedef{wv@clip_soft_prior_gps50_gain@hi}{13.6}
\@namedef{wv@clip_soft_prior_gps50_location_only_top_1@v}{59.9}
\@namedef{wv@clip_soft_prior_gps50_location_only_top_1@ci}{54.3 to 65.4}
\@namedef{wv@clip_soft_prior_gps50_location_only_top_1@lo}{54.3}
\@namedef{wv@clip_soft_prior_gps50_location_only_top_1@hi}{65.4}
\@namedef{wv@clip_soft_prior_gps50_top_1@v}{94.4}
\@namedef{wv@clip_soft_prior_gps50_top_1@ci}{93.2 to 95.6}
\@namedef{wv@clip_soft_prior_gps50_top_1@lo}{93.2}
\@namedef{wv@clip_soft_prior_gps50_top_1@hi}{95.6}
\@namedef{wv@clip_soft_prior_gps50_w0.005_top_1@v}{84.4}
\@namedef{wv@clip_soft_prior_gps50_w0.01_top_1@v}{86.0}
\@namedef{wv@clip_soft_prior_gps50_w0.02_top_1@v}{87.7}
\@namedef{wv@clip_soft_prior_gps50_w0.05_top_1@v}{91.1}
\@namedef{wv@clip_soft_prior_gps50_w0.1_top_1@v}{93.3}
\@namedef{wv@clip_soft_prior_gps50_w0.2_top_1@v}{94.4}
\@namedef{wv@clip_soft_prior_gps50_w0.5_top_1@v}{91.6}
\@namedef{wv@clip_soft_prior_gps50_w0_top_1@v}{82.8}
\@namedef{wv@clip_soft_prior_gps50_w10_top_1@v}{62.4}
\@namedef{wv@clip_soft_prior_gps50_w1_top_1@v}{82.6}
\@namedef{wv@clip_soft_prior_gps50_w20_top_1@v}{61.2}
\@namedef{wv@clip_soft_prior_gps50_w2_top_1@v}{71.7}
\@namedef{wv@clip_soft_prior_gps50_w5_top_1@v}{64.7}
\@namedef{wv@clip_soft_prior_none_top_1@v}{82.8}
\@namedef{wv@clip_soft_prior_none_top_1@ci}{80.6 to 85.0}
\@namedef{wv@clip_soft_prior_none_top_1@lo}{80.6}
\@namedef{wv@clip_soft_prior_none_top_1@hi}{85.0}
\@namedef{wv@clip_top_1@v}{82.9}
\@namedef{wv@clip_top_1@ci}{80.7 to 85.0}
\@namedef{wv@clip_top_1@lo}{80.7}
\@namedef{wv@clip_top_1@hi}{85.0}
\@namedef{wv@cv_cosine_top_1@v}{81.8}
\@namedef{wv@cv_cosine_top_1@ci}{79.5 to 84.0}
\@namedef{wv@cv_cosine_top_1@lo}{79.5}
\@namedef{wv@cv_cosine_top_1@hi}{84.0}
\@namedef{wv@cv_cosine_top_5@v}{89.0}
\@namedef{wv@cv_cosine_top_5@ci}{87.1 to 90.7}
\@namedef{wv@cv_cosine_top_5@lo}{87.1}
\@namedef{wv@cv_cosine_top_5@hi}{90.7}
\@namedef{wv@cv_disk-lightglue_top_1@v}{84.4}
\@namedef{wv@cv_disk-lightglue_top_1@ci}{82.1 to 86.3}
\@namedef{wv@cv_disk-lightglue_top_1@lo}{82.1}
\@namedef{wv@cv_disk-lightglue_top_1@hi}{86.3}
\@namedef{wv@cv_disk-lightglue_top_5@v}{89.6}
\@namedef{wv@cv_disk-lightglue_top_5@ci}{87.7 to 91.3}
\@namedef{wv@cv_disk-lightglue_top_5@lo}{87.7}
\@namedef{wv@cv_disk-lightglue_top_5@hi}{91.3}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_1_gain@v}{2.5}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_1_gain@ci}{1.3 to 3.9}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_1_gain@lo}{1.3}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_1_gain@hi}{3.9}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_1_losses@v}{8}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_1_p_value@v}{$1.5\times10^{-5}$}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_1_wins@v}{37}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_5_gain@v}{0.6}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_5_gain@ci}{0.1 to 1.3}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_5_gain@lo}{0.1}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_5_gain@hi}{1.3}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_5_losses@v}{2}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_5_p_value@v}{0.065}
\@namedef{wv@cv_disk-lightglue_vs_cosine_top_5_wins@v}{9}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_1_gain@v}{2.2}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_1_gain@ci}{1.0 to 3.5}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_1_gain@lo}{1.0}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_1_gain@hi}{3.5}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_1_losses@v}{8}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_1_p_value@v}{$6.9\times10^{-5}$}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_1_wins@v}{34}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_5_gain@v}{0.5}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_5_gain@ci}{0.0 to 1.2}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_5_gain@lo}{0.0}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_5_gain@hi}{1.2}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_5_losses@v}{2}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_5_p_value@v}{0.11}
\@namedef{wv@cv_disk-lightglue_vs_sift_top_5_wins@v}{8}
\@namedef{wv@cv_k50_cosine_top_1@v}{81.8}
\@namedef{wv@cv_k50_cosine_top_1@ci}{79.5 to 84.0}
\@namedef{wv@cv_k50_cosine_top_1@lo}{79.5}
\@namedef{wv@cv_k50_cosine_top_1@hi}{84.0}
\@namedef{wv@cv_k50_cosine_top_5@v}{89.0}
\@namedef{wv@cv_k50_cosine_top_5@ci}{87.1 to 90.7}
\@namedef{wv@cv_k50_cosine_top_5@lo}{87.1}
\@namedef{wv@cv_k50_cosine_top_5@hi}{90.7}
\@namedef{wv@cv_k50_disk-lightglue_fold_0_weight@v}{0.3}
\@namedef{wv@cv_k50_disk-lightglue_fold_1_weight@v}{0.2}
\@namedef{wv@cv_k50_disk-lightglue_fold_2_weight@v}{0.3}
\@namedef{wv@cv_k50_disk-lightglue_fold_3_weight@v}{0.3}
\@namedef{wv@cv_k50_disk-lightglue_fold_4_weight@v}{0.3}
\@namedef{wv@cv_k50_disk-lightglue_top_1@v}{85.2}
\@namedef{wv@cv_k50_disk-lightglue_top_1@ci}{83.1 to 87.1}
\@namedef{wv@cv_k50_disk-lightglue_top_1@lo}{83.1}
\@namedef{wv@cv_k50_disk-lightglue_top_1@hi}{87.1}
\@namedef{wv@cv_k50_disk-lightglue_top_5@v}{90.5}
\@namedef{wv@cv_k50_disk-lightglue_top_5@ci}{88.7 to 92.1}
\@namedef{wv@cv_k50_disk-lightglue_top_5@lo}{88.7}
\@namedef{wv@cv_k50_disk-lightglue_top_5@hi}{92.1}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_1_gain@v}{3.4}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_1_gain@ci}{1.7 to 5.2}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_1_gain@lo}{1.7}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_1_gain@hi}{5.2}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_1_losses@v}{15}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_1_p_value@v}{$2.6\times10^{-6}$}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_1_wins@v}{54}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_5_gain@v}{1.5}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_5_gain@ci}{0.6 to 2.4}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_5_gain@lo}{0.6}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_5_gain@hi}{2.4}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_5_losses@v}{5}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_5_p_value@v}{0.0015}
\@namedef{wv@cv_k50_disk-lightglue_vs_cosine_top_5_wins@v}{22}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_1_gain@v}{3.2}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_1_gain@ci}{1.7 to 4.8}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_1_gain@lo}{1.7}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_1_gain@hi}{4.8}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_1_losses@v}{14}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_1_p_value@v}{$4.5\times10^{-6}$}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_1_wins@v}{51}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_5_gain@v}{1.3}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_5_gain@ci}{0.5 to 2.2}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_5_gain@lo}{0.5}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_5_gain@hi}{2.2}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_5_losses@v}{5}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_5_p_value@v}{0.0041}
\@namedef{wv@cv_k50_disk-lightglue_vs_sift_top_5_wins@v}{20}
\@namedef{wv@cv_k50_queries@v}{1157}
\@namedef{wv@cv_k50_sift_fold_0_weight@v}{0.02}
\@namedef{wv@cv_k50_sift_fold_1_weight@v}{0.05}
\@namedef{wv@cv_k50_sift_fold_2_weight@v}{0.02}
\@namedef{wv@cv_k50_sift_fold_3_weight@v}{0.1}
\@namedef{wv@cv_k50_sift_fold_4_weight@v}{0.05}
\@namedef{wv@cv_k50_sift_top_1@v}{82.0}
\@namedef{wv@cv_k50_sift_top_1@ci}{79.7 to 84.1}
\@namedef{wv@cv_k50_sift_top_1@lo}{79.7}
\@namedef{wv@cv_k50_sift_top_1@hi}{84.1}
\@namedef{wv@cv_k50_sift_top_5@v}{89.2}
\@namedef{wv@cv_k50_sift_top_5@ci}{87.3 to 90.9}
\@namedef{wv@cv_k50_sift_top_5@lo}{87.3}
\@namedef{wv@cv_k50_sift_top_5@hi}{90.9}
\@namedef{wv@cv_k50_sift_vs_cosine_top_1_gain@v}{0.2}
\@namedef{wv@cv_k50_sift_vs_cosine_top_1_gain@ci}{$-$0.5 to 0.9}
\@namedef{wv@cv_k50_sift_vs_cosine_top_1_gain@lo}{$-$0.5}
\@namedef{wv@cv_k50_sift_vs_cosine_top_1_gain@hi}{0.9}
\@namedef{wv@cv_k50_sift_vs_cosine_top_1_losses@v}{6}
\@namedef{wv@cv_k50_sift_vs_cosine_top_1_p_value@v}{0.79}
\@namedef{wv@cv_k50_sift_vs_cosine_top_1_wins@v}{8}
\@namedef{wv@cv_k50_sift_vs_cosine_top_5_gain@v}{0.2}
\@namedef{wv@cv_k50_sift_vs_cosine_top_5_gain@ci}{$-$0.2 to 0.6}
\@namedef{wv@cv_k50_sift_vs_cosine_top_5_gain@lo}{$-$0.2}
\@namedef{wv@cv_k50_sift_vs_cosine_top_5_gain@hi}{0.6}
\@namedef{wv@cv_k50_sift_vs_cosine_top_5_losses@v}{1}
\@namedef{wv@cv_k50_sift_vs_cosine_top_5_p_value@v}{0.62}
\@namedef{wv@cv_k50_sift_vs_cosine_top_5_wins@v}{3}
\@namedef{wv@cv_k50_statues@v}{181}
\@namedef{wv@cv_loftr_top_1@v}{85.5}
\@namedef{wv@cv_loftr_top_1@ci}{83.3 to 87.4}
\@namedef{wv@cv_loftr_top_1@lo}{83.3}
\@namedef{wv@cv_loftr_top_1@hi}{87.4}
\@namedef{wv@cv_loftr_top_5@v}{89.3}
\@namedef{wv@cv_loftr_top_5@ci}{87.4 to 90.9}
\@namedef{wv@cv_loftr_top_5@lo}{87.4}
\@namedef{wv@cv_loftr_top_5@hi}{90.9}
\@namedef{wv@cv_loftr_vs_cosine_top_1_gain@v}{3.6}
\@namedef{wv@cv_loftr_vs_cosine_top_1_gain@ci}{2.2 to 5.2}
\@namedef{wv@cv_loftr_vs_cosine_top_1_gain@lo}{2.2}
\@namedef{wv@cv_loftr_vs_cosine_top_1_gain@hi}{5.2}
\@namedef{wv@cv_loftr_vs_cosine_top_1_losses@v}{9}
\@namedef{wv@cv_loftr_vs_cosine_top_1_p_value@v}{$3.1\times10^{-8}$}
\@namedef{wv@cv_loftr_vs_cosine_top_1_wins@v}{51}
\@namedef{wv@cv_loftr_vs_cosine_top_5_gain@v}{0.3}
\@namedef{wv@cv_loftr_vs_cosine_top_5_gain@ci}{$-$0.3 to 0.8}
\@namedef{wv@cv_loftr_vs_cosine_top_5_gain@lo}{$-$0.3}
\@namedef{wv@cv_loftr_vs_cosine_top_5_gain@hi}{0.8}
\@namedef{wv@cv_loftr_vs_cosine_top_5_losses@v}{3}
\@namedef{wv@cv_loftr_vs_cosine_top_5_p_value@v}{0.51}
\@namedef{wv@cv_loftr_vs_cosine_top_5_wins@v}{6}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_1_gain@v}{1.1}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_1_gain@ci}{0.1 to 2.2}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_1_gain@lo}{0.1}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_1_gain@hi}{2.2}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_1_losses@v}{13}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_1_p_value@v}{0.053}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_1_wins@v}{26}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_5_gain@v}{$-$0.3}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_5_gain@ci}{$-$1.0 to 0.2}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_5_gain@lo}{$-$1.0}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_5_gain@hi}{0.2}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_5_losses@v}{7}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_5_p_value@v}{0.34}
\@namedef{wv@cv_loftr_vs_disk-lightglue_top_5_wins@v}{3}
\@namedef{wv@cv_loftr_vs_sift_top_1_gain@v}{3.4}
\@namedef{wv@cv_loftr_vs_sift_top_1_gain@ci}{2.0 to 4.8}
\@namedef{wv@cv_loftr_vs_sift_top_1_gain@lo}{2.0}
\@namedef{wv@cv_loftr_vs_sift_top_1_gain@hi}{4.8}
\@namedef{wv@cv_loftr_vs_sift_top_1_losses@v}{12}
\@namedef{wv@cv_loftr_vs_sift_top_1_p_value@v}{$7.5\times10^{-7}$}
\@namedef{wv@cv_loftr_vs_sift_top_1_wins@v}{51}
\@namedef{wv@cv_loftr_vs_sift_top_5_gain@v}{0.2}
\@namedef{wv@cv_loftr_vs_sift_top_5_gain@ci}{$-$0.2 to 0.6}
\@namedef{wv@cv_loftr_vs_sift_top_5_gain@lo}{$-$0.2}
\@namedef{wv@cv_loftr_vs_sift_top_5_gain@hi}{0.6}
\@namedef{wv@cv_loftr_vs_sift_top_5_losses@v}{2}
\@namedef{wv@cv_loftr_vs_sift_top_5_p_value@v}{0.69}
\@namedef{wv@cv_loftr_vs_sift_top_5_wins@v}{4}
\@namedef{wv@cv_queries@v}{1157}
\@namedef{wv@cv_sift_top_1@v}{82.1}
\@namedef{wv@cv_sift_top_1@ci}{79.8 to 84.2}
\@namedef{wv@cv_sift_top_1@lo}{79.8}
\@namedef{wv@cv_sift_top_1@hi}{84.2}
\@namedef{wv@cv_sift_top_5@v}{89.1}
\@namedef{wv@cv_sift_top_5@ci}{87.2 to 90.8}
\@namedef{wv@cv_sift_top_5@lo}{87.2}
\@namedef{wv@cv_sift_top_5@hi}{90.8}
\@namedef{wv@cv_sift_vs_cosine_top_1_gain@v}{0.3}
\@namedef{wv@cv_sift_vs_cosine_top_1_gain@ci}{$-$0.4 to 0.9}
\@namedef{wv@cv_sift_vs_cosine_top_1_gain@lo}{$-$0.4}
\@namedef{wv@cv_sift_vs_cosine_top_1_gain@hi}{0.9}
\@namedef{wv@cv_sift_vs_cosine_top_1_losses@v}{5}
\@namedef{wv@cv_sift_vs_cosine_top_1_p_value@v}{0.58}
\@namedef{wv@cv_sift_vs_cosine_top_1_wins@v}{8}
\@namedef{wv@cv_sift_vs_cosine_top_5_gain@v}{0.1}
\@namedef{wv@cv_sift_vs_cosine_top_5_gain@ci}{$-$0.2 to 0.4}
\@namedef{wv@cv_sift_vs_cosine_top_5_gain@lo}{$-$0.2}
\@namedef{wv@cv_sift_vs_cosine_top_5_gain@hi}{0.4}
\@namedef{wv@cv_sift_vs_cosine_top_5_losses@v}{1}
\@namedef{wv@cv_sift_vs_cosine_top_5_p_value@v}{1}
\@namedef{wv@cv_sift_vs_cosine_top_5_wins@v}{2}
\@namedef{wv@cv_statues@v}{181}
\@namedef{wv@dinov2_families_count@v}{34}
\@namedef{wv@dinov2_families_error_share@v}{13.8}
\@namedef{wv@dinov2_families_error_share@ci}{6.5 to 21.9}
\@namedef{wv@dinov2_families_error_share@lo}{6.5}
\@namedef{wv@dinov2_families_error_share@hi}{21.9}
\@namedef{wv@dinov2_families_errors@v}{116}
\@namedef{wv@dinov2_families_inside_error_rate@v}{6.9}
\@namedef{wv@dinov2_families_inside_error_rate@ci}{4.8 to 9.3}
\@namedef{wv@dinov2_families_inside_error_rate@lo}{4.8}
\@namedef{wv@dinov2_families_inside_error_rate@hi}{9.3}
\@namedef{wv@dinov2_families_outside_error_rate@v}{6.8}
\@namedef{wv@dinov2_families_outside_error_rate@ci}{5.3 to 8.4}
\@namedef{wv@dinov2_families_outside_error_rate@lo}{5.3}
\@namedef{wv@dinov2_families_outside_error_rate@hi}{8.4}
\@namedef{wv@dinov2_families_statue_share@v}{30.7}
\@namedef{wv@dinov2_families_statues@v}{94}
\@namedef{wv@dinov2_geo_minus_random_pool_10@v}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_10@ci}{$-$1.4 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_10@lo}{$-$1.4}
\@namedef{wv@dinov2_geo_minus_random_pool_10@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_100@v}{$-$0.5}
\@namedef{wv@dinov2_geo_minus_random_pool_100@ci}{$-$1.0 to 0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_100@lo}{$-$1.0}
\@namedef{wv@dinov2_geo_minus_random_pool_100@hi}{0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_150@v}{$-$0.5}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_150@ci}{$-$1.1 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_150@lo}{$-$1.1}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_150@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_50@v}{$-$0.5}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_50@ci}{$-$1.0 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_50@lo}{$-$1.0}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_50@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_9@v}{$-$0.5}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_9@ci}{$-$1.0 to 0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_9@lo}{$-$1.0}
\@namedef{wv@dinov2_geo_minus_random_pool_100_noise_9@hi}{0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_150@v}{$-$0.4}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_150@ci}{$-$0.9 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_150@lo}{$-$0.9}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_150@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_50@v}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_50@ci}{$-$1.2 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_50@lo}{$-$1.2}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_50@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_9@v}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_9@ci}{$-$1.4 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_9@lo}{$-$1.4}
\@namedef{wv@dinov2_geo_minus_random_pool_10_noise_9@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_15@v}{$-$0.8}
\@namedef{wv@dinov2_geo_minus_random_pool_15@ci}{$-$1.4 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_15@lo}{$-$1.4}
\@namedef{wv@dinov2_geo_minus_random_pool_15@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_150@v}{$-$0.4}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_150@ci}{$-$0.8 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_150@lo}{$-$0.8}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_150@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_50@v}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_50@ci}{$-$1.2 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_50@lo}{$-$1.2}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_50@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_9@v}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_9@ci}{$-$1.3 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_9@lo}{$-$1.3}
\@namedef{wv@dinov2_geo_minus_random_pool_15_noise_9@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_2@v}{$-$0.5}
\@namedef{wv@dinov2_geo_minus_random_pool_2@ci}{$-$1.0 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_2@lo}{$-$1.0}
\@namedef{wv@dinov2_geo_minus_random_pool_2@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_20@v}{$-$0.8}
\@namedef{wv@dinov2_geo_minus_random_pool_20@ci}{$-$1.4 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_20@lo}{$-$1.4}
\@namedef{wv@dinov2_geo_minus_random_pool_20@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_200@v}{$-$0.4}
\@namedef{wv@dinov2_geo_minus_random_pool_200@ci}{$-$0.6 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_200@lo}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_200@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_150@v}{$-$0.4}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_150@ci}{$-$0.6 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_150@lo}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_150@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_50@v}{$-$0.4}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_50@ci}{$-$0.6 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_50@lo}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_50@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_9@v}{$-$0.4}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_9@ci}{$-$0.6 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_9@lo}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_200_noise_9@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_150@v}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_150@ci}{$-$1.1 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_150@lo}{$-$1.1}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_150@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_50@v}{$-$0.8}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_50@ci}{$-$1.4 to $-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_50@lo}{$-$1.4}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_50@hi}{$-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_9@v}{$-$0.8}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_9@ci}{$-$1.4 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_9@lo}{$-$1.4}
\@namedef{wv@dinov2_geo_minus_random_pool_20_noise_9@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_294@v}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294@ci}{0.0 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294@lo}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_150@v}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_150@ci}{0.0 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_150@lo}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_150@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_50@v}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_50@ci}{0.0 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_50@lo}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_50@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_9@v}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_9@ci}{0.0 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_9@lo}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_294_noise_9@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_150@v}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_150@ci}{$-$0.6 to 0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_150@lo}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_150@hi}{0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_50@v}{$-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_50@ci}{$-$0.7 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_50@lo}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_50@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_9@v}{$-$0.5}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_9@ci}{$-$0.9 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_9@lo}{$-$0.9}
\@namedef{wv@dinov2_geo_minus_random_pool_2_noise_9@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_3@v}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_3@ci}{$-$1.2 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_3@lo}{$-$1.2}
\@namedef{wv@dinov2_geo_minus_random_pool_3@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_150@v}{$-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_150@ci}{$-$0.6 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_150@lo}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_150@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_50@v}{$-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_50@ci}{$-$0.7 to 0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_50@lo}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_50@hi}{0.0}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_9@v}{$-$0.5}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_9@ci}{$-$1.0 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_9@lo}{$-$1.0}
\@namedef{wv@dinov2_geo_minus_random_pool_3_noise_9@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_5@v}{$-$0.9}
\@namedef{wv@dinov2_geo_minus_random_pool_5@ci}{$-$1.5 to $-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_5@lo}{$-$1.5}
\@namedef{wv@dinov2_geo_minus_random_pool_5@hi}{$-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_50@v}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_50@ci}{$-$1.2 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_50@lo}{$-$1.2}
\@namedef{wv@dinov2_geo_minus_random_pool_50@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_150@v}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_150@ci}{$-$1.1 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_150@lo}{$-$1.1}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_150@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_50@v}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_50@ci}{$-$1.2 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_50@lo}{$-$1.2}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_50@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_9@v}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_9@ci}{$-$1.3 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_9@lo}{$-$1.3}
\@namedef{wv@dinov2_geo_minus_random_pool_50_noise_9@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_150@v}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_150@ci}{$-$1.1 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_150@lo}{$-$1.1}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_150@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_50@v}{$-$0.6}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_50@ci}{$-$1.1 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_50@lo}{$-$1.1}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_50@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_9@v}{$-$0.9}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_9@ci}{$-$1.5 to $-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_9@lo}{$-$1.5}
\@namedef{wv@dinov2_geo_minus_random_pool_5_noise_9@hi}{$-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_8@v}{$-$0.7}
\@namedef{wv@dinov2_geo_minus_random_pool_8@ci}{$-$1.4 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_8@lo}{$-$1.4}
\@namedef{wv@dinov2_geo_minus_random_pool_8@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_150@v}{$-$0.5}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_150@ci}{$-$1.0 to $-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_150@lo}{$-$1.0}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_150@hi}{$-$0.1}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_50@v}{$-$0.8}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_50@ci}{$-$1.3 to $-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_50@lo}{$-$1.3}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_50@hi}{$-$0.3}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_9@v}{$-$0.8}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_9@ci}{$-$1.5 to $-$0.2}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_9@lo}{$-$1.5}
\@namedef{wv@dinov2_geo_minus_random_pool_8_noise_9@hi}{$-$0.2}
\@namedef{wv@dinov2_geo_permutation_mean_null@v}{0.1}
\@namedef{wv@dinov2_geo_permutation_mean_null@ci}{$-$0.3 to 0.4}
\@namedef{wv@dinov2_geo_permutation_mean_null@lo}{$-$0.3}
\@namedef{wv@dinov2_geo_permutation_mean_null@hi}{0.4}
\@namedef{wv@dinov2_geo_permutation_mean_observed@v}{$-$0.8}
\@namedef{wv@dinov2_geo_permutation_mean_p_value@v}{0.005}
\@namedef{wv@dinov2_geo_permutation_permutations@v}{200}
\@namedef{wv@dinov2_geo_permutation_pool_10_null_mean@v}{0.2}
\@namedef{wv@dinov2_geo_permutation_pool_10_null_mean@ci}{$-$0.3 to 0.6}
\@namedef{wv@dinov2_geo_permutation_pool_10_null_mean@lo}{$-$0.3}
\@namedef{wv@dinov2_geo_permutation_pool_10_null_mean@hi}{0.6}
\@namedef{wv@dinov2_geo_permutation_pool_10_p_value@v}{0.005}
\@namedef{wv@dinov2_geo_permutation_pool_20_null_mean@v}{0.0}
\@namedef{wv@dinov2_geo_permutation_pool_20_null_mean@ci}{$-$0.4 to 0.5}
\@namedef{wv@dinov2_geo_permutation_pool_20_null_mean@lo}{$-$0.4}
\@namedef{wv@dinov2_geo_permutation_pool_20_null_mean@hi}{0.5}
\@namedef{wv@dinov2_geo_permutation_pool_20_p_value@v}{0.005}
\@namedef{wv@dinov2_geo_permutation_pool_5_null_mean@v}{$-$0.1}
\@namedef{wv@dinov2_geo_permutation_pool_5_null_mean@ci}{$-$0.5 to 0.3}
\@namedef{wv@dinov2_geo_permutation_pool_5_null_mean@lo}{$-$0.5}
\@namedef{wv@dinov2_geo_permutation_pool_5_null_mean@hi}{0.3}
\@namedef{wv@dinov2_geo_permutation_pool_5_p_value@v}{0.005}
\@namedef{wv@dinov2_groups_changed_queries@v}{3}
\@namedef{wv@dinov2_groups_merged_gain@v}{0.2}
\@namedef{wv@dinov2_groups_merged_gain@ci}{0.0 to 0.5}
\@namedef{wv@dinov2_groups_merged_gain@lo}{0.0}
\@namedef{wv@dinov2_groups_merged_gain@hi}{0.5}
\@namedef{wv@dinov2_groups_merged_top_1@v}{93.3}
\@namedef{wv@dinov2_groups_merged_top_1@ci}{92.0 to 94.5}
\@namedef{wv@dinov2_groups_merged_top_1@lo}{92.0}
\@namedef{wv@dinov2_groups_merged_top_1@hi}{94.5}
\@namedef{wv@dinov2_minus_clip_top_1@v}{10.2}
\@namedef{wv@dinov2_minus_clip_top_1@ci}{8.4 to 12.2}
\@namedef{wv@dinov2_minus_clip_top_1@lo}{8.4}
\@namedef{wv@dinov2_minus_clip_top_1@hi}{12.2}
\@namedef{wv@dinov2_minus_dinov3_top_1@v}{$-$1.3}
\@namedef{wv@dinov2_minus_dinov3_top_1@ci}{$-$2.2 to $-$0.4}
\@namedef{wv@dinov2_minus_dinov3_top_1@lo}{$-$2.2}
\@namedef{wv@dinov2_minus_dinov3_top_1@hi}{$-$0.4}
\@namedef{wv@dinov2_minus_siglip2_top_1@v}{2.0}
\@namedef{wv@dinov2_minus_siglip2_top_1@ci}{0.8 to 3.2}
\@namedef{wv@dinov2_minus_siglip2_top_1@lo}{0.8}
\@namedef{wv@dinov2_minus_siglip2_top_1@hi}{3.2}
\@namedef{wv@dinov2_photographer_attributable@v}{2.6}
\@namedef{wv@dinov2_photographer_attributable@ci}{1.0 to 4.3}
\@namedef{wv@dinov2_photographer_attributable@lo}{1.0}
\@namedef{wv@dinov2_photographer_attributable@hi}{4.3}
\@namedef{wv@dinov2_photographer_raw_gap@v}{12.4}
\@namedef{wv@dinov2_photographer_raw_gap@ci}{9.2 to 15.8}
\@namedef{wv@dinov2_photographer_raw_gap@lo}{9.2}
\@namedef{wv@dinov2_photographer_raw_gap@hi}{15.8}
\@namedef{wv@dinov2_photographer_reference_cost@v}{9.7}
\@namedef{wv@dinov2_photographer_reference_cost@ci}{7.2 to 12.7}
\@namedef{wv@dinov2_photographer_reference_cost@lo}{7.2}
\@namedef{wv@dinov2_photographer_reference_cost@hi}{12.7}
\@namedef{wv@dinov2_points_per_doubling@v}{$-$0.8}
\@namedef{wv@dinov2_points_per_doubling@ci}{$-$1.0 to $-$0.6}
\@namedef{wv@dinov2_points_per_doubling@lo}{$-$1.0}
\@namedef{wv@dinov2_points_per_doubling@hi}{$-$0.6}
\@namedef{wv@dinov2_reject_cosine_auroc@v}{0.896}
\@namedef{wv@dinov2_reject_cosine_auroc@ci}{0.883 to 0.909}
\@namedef{wv@dinov2_reject_cosine_auroc@lo}{0.883}
\@namedef{wv@dinov2_reject_cosine_auroc@hi}{0.909}
\@namedef{wv@dinov2_reject_cosine_false_acceptance_90@v}{38.3}
\@namedef{wv@dinov2_reject_cosine_known_acceptance_90@v}{90.0}
\@namedef{wv@dinov2_reject_knn_auroc@v}{0.637}
\@namedef{wv@dinov2_reject_knn_auroc@ci}{0.611 to 0.665}
\@namedef{wv@dinov2_reject_knn_auroc@lo}{0.611}
\@namedef{wv@dinov2_reject_knn_auroc@hi}{0.665}
\@namedef{wv@dinov2_reject_knn_false_acceptance_90@v}{82.2}
\@namedef{wv@dinov2_reject_knn_known_acceptance_90@v}{90.0}
\@namedef{wv@dinov2_reject_knn_minus_cosine_auroc@v}{$-$0.259}
\@namedef{wv@dinov2_reject_knn_minus_cosine_auroc@ci}{$-$0.281 to $-$0.236}
\@namedef{wv@dinov2_reject_knn_minus_cosine_auroc@lo}{$-$0.281}
\@namedef{wv@dinov2_reject_knn_minus_cosine_auroc@hi}{$-$0.236}
\@namedef{wv@dinov2_reject_margin_auroc@v}{0.927}
\@namedef{wv@dinov2_reject_margin_auroc@ci}{0.914 to 0.940}
\@namedef{wv@dinov2_reject_margin_auroc@lo}{0.914}
\@namedef{wv@dinov2_reject_margin_auroc@hi}{0.940}
\@namedef{wv@dinov2_reject_margin_false_acceptance_90@v}{19.6}
\@namedef{wv@dinov2_reject_margin_known_acceptance_90@v}{89.9}
\@namedef{wv@dinov2_reject_margin_minus_cosine_auroc@v}{0.032}
\@namedef{wv@dinov2_reject_margin_minus_cosine_auroc@ci}{0.020 to 0.043}
\@namedef{wv@dinov2_reject_margin_minus_cosine_auroc@lo}{0.020}
\@namedef{wv@dinov2_reject_margin_minus_cosine_auroc@hi}{0.043}
\@namedef{wv@dinov2_soft_prior_gps10_fold_0_weight@v}{2}
\@namedef{wv@dinov2_soft_prior_gps10_fold_1_weight@v}{2}
\@namedef{wv@dinov2_soft_prior_gps10_fold_2_weight@v}{2}
\@namedef{wv@dinov2_soft_prior_gps10_fold_3_weight@v}{2}
\@namedef{wv@dinov2_soft_prior_gps10_fold_4_weight@v}{2}
\@namedef{wv@dinov2_soft_prior_gps10_gain@v}{5.7}
\@namedef{wv@dinov2_soft_prior_gps10_gain@ci}{4.6 to 6.9}
\@namedef{wv@dinov2_soft_prior_gps10_gain@lo}{4.6}
\@namedef{wv@dinov2_soft_prior_gps10_gain@hi}{6.9}
\@namedef{wv@dinov2_soft_prior_gps10_location_only_top_1@v}{90.9}
\@namedef{wv@dinov2_soft_prior_gps10_location_only_top_1@ci}{88.0 to 93.6}
\@namedef{wv@dinov2_soft_prior_gps10_location_only_top_1@lo}{88.0}
\@namedef{wv@dinov2_soft_prior_gps10_location_only_top_1@hi}{93.6}
\@namedef{wv@dinov2_soft_prior_gps10_top_1@v}{99.1}
\@namedef{wv@dinov2_soft_prior_gps10_top_1@ci}{98.6 to 99.6}
\@namedef{wv@dinov2_soft_prior_gps10_top_1@lo}{98.6}
\@namedef{wv@dinov2_soft_prior_gps10_top_1@hi}{99.6}
\@namedef{wv@dinov2_soft_prior_gps10_w0.005_top_1@v}{93.6}
\@namedef{wv@dinov2_soft_prior_gps10_w0.01_top_1@v}{93.7}
\@namedef{wv@dinov2_soft_prior_gps10_w0.02_top_1@v}{94.0}
\@namedef{wv@dinov2_soft_prior_gps10_w0.05_top_1@v}{94.8}
\@namedef{wv@dinov2_soft_prior_gps10_w0.1_top_1@v}{95.7}
\@namedef{wv@dinov2_soft_prior_gps10_w0.2_top_1@v}{96.8}
\@namedef{wv@dinov2_soft_prior_gps10_w0.5_top_1@v}{98.4}
\@namedef{wv@dinov2_soft_prior_gps10_w0_top_1@v}{93.4}
\@namedef{wv@dinov2_soft_prior_gps10_w10_top_1@v}{98.0}
\@namedef{wv@dinov2_soft_prior_gps10_w1_top_1@v}{98.9}
\@namedef{wv@dinov2_soft_prior_gps10_w20_top_1@v}{95.5}
\@namedef{wv@dinov2_soft_prior_gps10_w2_top_1@v}{99.1}
\@namedef{wv@dinov2_soft_prior_gps10_w5_top_1@v}{99.0}
\@namedef{wv@dinov2_soft_prior_gps25_fold_0_weight@v}{1}
\@namedef{wv@dinov2_soft_prior_gps25_fold_1_weight@v}{1}
\@namedef{wv@dinov2_soft_prior_gps25_fold_2_weight@v}{1}
\@namedef{wv@dinov2_soft_prior_gps25_fold_3_weight@v}{1}
\@namedef{wv@dinov2_soft_prior_gps25_fold_4_weight@v}{1}
\@namedef{wv@dinov2_soft_prior_gps25_gain@v}{5.2}
\@namedef{wv@dinov2_soft_prior_gps25_gain@ci}{4.2 to 6.4}
\@namedef{wv@dinov2_soft_prior_gps25_gain@lo}{4.2}
\@namedef{wv@dinov2_soft_prior_gps25_gain@hi}{6.4}
\@namedef{wv@dinov2_soft_prior_gps25_location_only_top_1@v}{75.1}
\@namedef{wv@dinov2_soft_prior_gps25_location_only_top_1@ci}{70.7 to 79.4}
\@namedef{wv@dinov2_soft_prior_gps25_location_only_top_1@lo}{70.7}
\@namedef{wv@dinov2_soft_prior_gps25_location_only_top_1@hi}{79.4}
\@namedef{wv@dinov2_soft_prior_gps25_top_1@v}{98.7}
\@namedef{wv@dinov2_soft_prior_gps25_top_1@ci}{98.0 to 99.3}
\@namedef{wv@dinov2_soft_prior_gps25_top_1@lo}{98.0}
\@namedef{wv@dinov2_soft_prior_gps25_top_1@hi}{99.3}
\@namedef{wv@dinov2_soft_prior_gps25_w0.005_top_1@v}{93.5}
\@namedef{wv@dinov2_soft_prior_gps25_w0.01_top_1@v}{93.7}
\@namedef{wv@dinov2_soft_prior_gps25_w0.02_top_1@v}{94.0}
\@namedef{wv@dinov2_soft_prior_gps25_w0.05_top_1@v}{94.7}
\@namedef{wv@dinov2_soft_prior_gps25_w0.1_top_1@v}{95.6}
\@namedef{wv@dinov2_soft_prior_gps25_w0.2_top_1@v}{96.6}
\@namedef{wv@dinov2_soft_prior_gps25_w0.5_top_1@v}{98.1}
\@namedef{wv@dinov2_soft_prior_gps25_w0_top_1@v}{93.4}
\@namedef{wv@dinov2_soft_prior_gps25_w10_top_1@v}{85.1}
\@namedef{wv@dinov2_soft_prior_gps25_w1_top_1@v}{98.7}
\@namedef{wv@dinov2_soft_prior_gps25_w20_top_1@v}{80.1}
\@namedef{wv@dinov2_soft_prior_gps25_w2_top_1@v}{98.3}
\@namedef{wv@dinov2_soft_prior_gps25_w5_top_1@v}{93.1}
\@namedef{wv@dinov2_soft_prior_gps50_fold_0_weight@v}{0.5}
\@namedef{wv@dinov2_soft_prior_gps50_fold_1_weight@v}{0.5}
\@namedef{wv@dinov2_soft_prior_gps50_fold_2_weight@v}{0.5}
\@namedef{wv@dinov2_soft_prior_gps50_fold_3_weight@v}{0.5}
\@namedef{wv@dinov2_soft_prior_gps50_fold_4_weight@v}{0.5}
\@namedef{wv@dinov2_soft_prior_gps50_gain@v}{4.1}
\@namedef{wv@dinov2_soft_prior_gps50_gain@ci}{3.1 to 5.1}
\@namedef{wv@dinov2_soft_prior_gps50_gain@lo}{3.1}
\@namedef{wv@dinov2_soft_prior_gps50_gain@hi}{5.1}
\@namedef{wv@dinov2_soft_prior_gps50_location_only_top_1@v}{60.2}
\@namedef{wv@dinov2_soft_prior_gps50_location_only_top_1@ci}{54.6 to 65.7}
\@namedef{wv@dinov2_soft_prior_gps50_location_only_top_1@lo}{54.6}
\@namedef{wv@dinov2_soft_prior_gps50_location_only_top_1@hi}{65.7}
\@namedef{wv@dinov2_soft_prior_gps50_top_1@v}{97.5}
\@namedef{wv@dinov2_soft_prior_gps50_top_1@ci}{96.7 to 98.2}
\@namedef{wv@dinov2_soft_prior_gps50_top_1@lo}{96.7}
\@namedef{wv@dinov2_soft_prior_gps50_top_1@hi}{98.2}
\@namedef{wv@dinov2_soft_prior_gps50_w0.005_top_1@v}{93.5}
\@namedef{wv@dinov2_soft_prior_gps50_w0.01_top_1@v}{93.7}
\@namedef{wv@dinov2_soft_prior_gps50_w0.02_top_1@v}{93.9}
\@namedef{wv@dinov2_soft_prior_gps50_w0.05_top_1@v}{94.5}
\@namedef{wv@dinov2_soft_prior_gps50_w0.1_top_1@v}{95.4}
\@namedef{wv@dinov2_soft_prior_gps50_w0.2_top_1@v}{96.4}
\@namedef{wv@dinov2_soft_prior_gps50_w0.5_top_1@v}{97.5}
\@namedef{wv@dinov2_soft_prior_gps50_w0_top_1@v}{93.4}
\@namedef{wv@dinov2_soft_prior_gps50_w10_top_1@v}{68.1}
\@namedef{wv@dinov2_soft_prior_gps50_w1_top_1@v}{97.3}
\@namedef{wv@dinov2_soft_prior_gps50_w20_top_1@v}{64.0}
\@namedef{wv@dinov2_soft_prior_gps50_w2_top_1@v}{92.1}
\@namedef{wv@dinov2_soft_prior_gps50_w5_top_1@v}{75.9}
\@namedef{wv@dinov2_soft_prior_none_top_1@v}{93.4}
\@namedef{wv@dinov2_soft_prior_none_top_1@ci}{92.1 to 94.6}
\@namedef{wv@dinov2_soft_prior_none_top_1@lo}{92.1}
\@namedef{wv@dinov2_soft_prior_none_top_1@hi}{94.6}
\@namedef{wv@dinov2_top_1@v}{93.1}
\@namedef{wv@dinov2_top_1@ci}{91.8 to 94.4}
\@namedef{wv@dinov2_top_1@lo}{91.8}
\@namedef{wv@dinov2_top_1@hi}{94.4}
\@namedef{wv@dinov3_families_count@v}{29}
\@namedef{wv@dinov3_families_error_share@v}{20.2}
\@namedef{wv@dinov3_families_error_share@ci}{10.2 to 31.2}
\@namedef{wv@dinov3_families_error_share@lo}{10.2}
\@namedef{wv@dinov3_families_error_share@hi}{31.2}
\@namedef{wv@dinov3_families_errors@v}{94}
\@namedef{wv@dinov3_families_inside_error_rate@v}{6.7}
\@namedef{wv@dinov3_families_inside_error_rate@ci}{4.1 to 9.6}
\@namedef{wv@dinov3_families_inside_error_rate@lo}{4.1}
\@namedef{wv@dinov3_families_inside_error_rate@hi}{9.6}
\@namedef{wv@dinov3_families_outside_error_rate@v}{5.1}
\@namedef{wv@dinov3_families_outside_error_rate@ci}{3.8 to 6.5}
\@namedef{wv@dinov3_families_outside_error_rate@lo}{3.8}
\@namedef{wv@dinov3_families_outside_error_rate@hi}{6.5}
\@namedef{wv@dinov3_families_statue_share@v}{26.5}
\@namedef{wv@dinov3_families_statues@v}{81}
\@namedef{wv@dinov3_geo_minus_random_pool_10@v}{$-$1.1}
\@namedef{wv@dinov3_geo_minus_random_pool_10@ci}{$-$1.9 to $-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_10@lo}{$-$1.9}
\@namedef{wv@dinov3_geo_minus_random_pool_10@hi}{$-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_100@v}{$-$1.1}
\@namedef{wv@dinov3_geo_minus_random_pool_100@ci}{$-$1.7 to $-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100@lo}{$-$1.7}
\@namedef{wv@dinov3_geo_minus_random_pool_100@hi}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_150@v}{$-$1.1}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_150@ci}{$-$1.6 to $-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_150@lo}{$-$1.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_150@hi}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_50@v}{$-$1.1}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_50@ci}{$-$1.6 to $-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_50@lo}{$-$1.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_50@hi}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_9@v}{$-$1.1}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_9@ci}{$-$1.6 to $-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_9@lo}{$-$1.6}
\@namedef{wv@dinov3_geo_minus_random_pool_100_noise_9@hi}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_150@v}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_150@ci}{$-$1.0 to $-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_150@lo}{$-$1.0}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_150@hi}{$-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_50@v}{$-$0.9}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_50@ci}{$-$1.6 to $-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_50@lo}{$-$1.6}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_50@hi}{$-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_9@v}{$-$1.2}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_9@ci}{$-$2.0 to $-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_9@lo}{$-$2.0}
\@namedef{wv@dinov3_geo_minus_random_pool_10_noise_9@hi}{$-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_15@v}{$-$1.4}
\@namedef{wv@dinov3_geo_minus_random_pool_15@ci}{$-$2.3 to $-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_15@lo}{$-$2.3}
\@namedef{wv@dinov3_geo_minus_random_pool_15@hi}{$-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_150@v}{$-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_150@ci}{$-$1.3 to $-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_150@lo}{$-$1.3}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_150@hi}{$-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_50@v}{$-$1.3}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_50@ci}{$-$2.0 to $-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_50@lo}{$-$2.0}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_50@hi}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_9@v}{$-$1.4}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_9@ci}{$-$2.3 to $-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_9@lo}{$-$2.3}
\@namedef{wv@dinov3_geo_minus_random_pool_15_noise_9@hi}{$-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_2@v}{$-$1.0}
\@namedef{wv@dinov3_geo_minus_random_pool_2@ci}{$-$1.7 to $-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_2@lo}{$-$1.7}
\@namedef{wv@dinov3_geo_minus_random_pool_2@hi}{$-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_20@v}{$-$1.6}
\@namedef{wv@dinov3_geo_minus_random_pool_20@ci}{$-$2.5 to $-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_20@lo}{$-$2.5}
\@namedef{wv@dinov3_geo_minus_random_pool_20@hi}{$-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_200@v}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_200@ci}{$-$0.9 to $-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_200@lo}{$-$0.9}
\@namedef{wv@dinov3_geo_minus_random_pool_200@hi}{$-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_150@v}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_150@ci}{$-$0.9 to $-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_150@lo}{$-$0.9}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_150@hi}{$-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_50@v}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_50@ci}{$-$0.9 to $-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_50@lo}{$-$0.9}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_50@hi}{$-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_9@v}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_9@ci}{$-$0.9 to $-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_9@lo}{$-$0.9}
\@namedef{wv@dinov3_geo_minus_random_pool_200_noise_9@hi}{$-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_150@v}{$-$1.3}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_150@ci}{$-$1.9 to $-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_150@lo}{$-$1.9}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_150@hi}{$-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_50@v}{$-$1.7}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_50@ci}{$-$2.5 to $-$1.0}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_50@lo}{$-$2.5}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_50@hi}{$-$1.0}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_9@v}{$-$1.6}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_9@ci}{$-$2.5 to $-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_9@lo}{$-$2.5}
\@namedef{wv@dinov3_geo_minus_random_pool_20_noise_9@hi}{$-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_294@v}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294@ci}{0.0 to 0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294@lo}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294@hi}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_150@v}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_150@ci}{0.0 to 0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_150@lo}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_150@hi}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_50@v}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_50@ci}{0.0 to 0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_50@lo}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_50@hi}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_9@v}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_9@ci}{0.0 to 0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_9@lo}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_294_noise_9@hi}{0.0}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_150@v}{$-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_150@ci}{$-$0.6 to $-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_150@lo}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_150@hi}{$-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_50@v}{$-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_50@ci}{$-$0.7 to $-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_50@lo}{$-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_50@hi}{$-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_9@v}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_9@ci}{$-$1.0 to $-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_9@lo}{$-$1.0}
\@namedef{wv@dinov3_geo_minus_random_pool_2_noise_9@hi}{$-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_3@v}{$-$1.0}
\@namedef{wv@dinov3_geo_minus_random_pool_3@ci}{$-$1.7 to $-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_3@lo}{$-$1.7}
\@namedef{wv@dinov3_geo_minus_random_pool_3@hi}{$-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_150@v}{$-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_150@ci}{$-$0.5 to $-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_150@lo}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_150@hi}{$-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_50@v}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_50@ci}{$-$0.8 to $-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_50@lo}{$-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_50@hi}{$-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_9@v}{$-$1.0}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_9@ci}{$-$1.7 to $-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_9@lo}{$-$1.7}
\@namedef{wv@dinov3_geo_minus_random_pool_3_noise_9@hi}{$-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_5@v}{$-$1.2}
\@namedef{wv@dinov3_geo_minus_random_pool_5@ci}{$-$2.0 to $-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_5@lo}{$-$2.0}
\@namedef{wv@dinov3_geo_minus_random_pool_5@hi}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_50@v}{$-$1.3}
\@namedef{wv@dinov3_geo_minus_random_pool_50@ci}{$-$2.0 to $-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_50@lo}{$-$2.0}
\@namedef{wv@dinov3_geo_minus_random_pool_50@hi}{$-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_150@v}{$-$1.2}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_150@ci}{$-$1.9 to $-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_150@lo}{$-$1.9}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_150@hi}{$-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_50@v}{$-$1.4}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_50@ci}{$-$2.1 to $-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_50@lo}{$-$2.1}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_50@hi}{$-$0.7}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_9@v}{$-$1.4}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_9@ci}{$-$2.2 to $-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_9@lo}{$-$2.2}
\@namedef{wv@dinov3_geo_minus_random_pool_50_noise_9@hi}{$-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_150@v}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_150@ci}{$-$1.0 to $-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_150@lo}{$-$1.0}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_150@hi}{$-$0.2}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_50@v}{$-$0.8}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_50@ci}{$-$1.2 to $-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_50@lo}{$-$1.2}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_50@hi}{$-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_9@v}{$-$1.3}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_9@ci}{$-$2.1 to $-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_9@lo}{$-$2.1}
\@namedef{wv@dinov3_geo_minus_random_pool_5_noise_9@hi}{$-$0.6}
\@namedef{wv@dinov3_geo_minus_random_pool_8@v}{$-$1.2}
\@namedef{wv@dinov3_geo_minus_random_pool_8@ci}{$-$2.0 to $-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_8@lo}{$-$2.0}
\@namedef{wv@dinov3_geo_minus_random_pool_8@hi}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_150@v}{$-$0.5}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_150@ci}{$-$0.9 to $-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_150@lo}{$-$0.9}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_150@hi}{$-$0.1}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_50@v}{$-$0.9}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_50@ci}{$-$1.6 to $-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_50@lo}{$-$1.6}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_50@hi}{$-$0.3}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_9@v}{$-$1.1}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_9@ci}{$-$1.9 to $-$0.4}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_9@lo}{$-$1.9}
\@namedef{wv@dinov3_geo_minus_random_pool_8_noise_9@hi}{$-$0.4}
\@namedef{wv@dinov3_geo_permutation_mean_null@v}{0.0}
\@namedef{wv@dinov3_geo_permutation_mean_null@ci}{$-$0.3 to 0.3}
\@namedef{wv@dinov3_geo_permutation_mean_null@lo}{$-$0.3}
\@namedef{wv@dinov3_geo_permutation_mean_null@hi}{0.3}
\@namedef{wv@dinov3_geo_permutation_mean_observed@v}{$-$1.3}
\@namedef{wv@dinov3_geo_permutation_mean_p_value@v}{0.005}
\@namedef{wv@dinov3_geo_permutation_permutations@v}{200}
\@namedef{wv@dinov3_geo_permutation_pool_10_null_mean@v}{0.1}
\@namedef{wv@dinov3_geo_permutation_pool_10_null_mean@ci}{$-$0.2 to 0.5}
\@namedef{wv@dinov3_geo_permutation_pool_10_null_mean@lo}{$-$0.2}
\@namedef{wv@dinov3_geo_permutation_pool_10_null_mean@hi}{0.5}
\@namedef{wv@dinov3_geo_permutation_pool_10_p_value@v}{0.005}
\@namedef{wv@dinov3_geo_permutation_pool_20_null_mean@v}{$-$0.1}
\@namedef{wv@dinov3_geo_permutation_pool_20_null_mean@ci}{$-$0.6 to 0.2}
\@namedef{wv@dinov3_geo_permutation_pool_20_null_mean@lo}{$-$0.6}
\@namedef{wv@dinov3_geo_permutation_pool_20_null_mean@hi}{0.2}
\@namedef{wv@dinov3_geo_permutation_pool_20_p_value@v}{0.005}
\@namedef{wv@dinov3_geo_permutation_pool_5_null_mean@v}{$-$0.1}
\@namedef{wv@dinov3_geo_permutation_pool_5_null_mean@ci}{$-$0.4 to 0.3}
\@namedef{wv@dinov3_geo_permutation_pool_5_null_mean@lo}{$-$0.4}
\@namedef{wv@dinov3_geo_permutation_pool_5_null_mean@hi}{0.3}
\@namedef{wv@dinov3_geo_permutation_pool_5_p_value@v}{0.005}
\@namedef{wv@dinov3_groups_changed_queries@v}{3}
\@namedef{wv@dinov3_groups_merged_gain@v}{0.2}
\@namedef{wv@dinov3_groups_merged_gain@ci}{0.0 to 0.5}
\@namedef{wv@dinov3_groups_merged_gain@lo}{0.0}
\@namedef{wv@dinov3_groups_merged_gain@hi}{0.5}
\@namedef{wv@dinov3_groups_merged_top_1@v}{94.6}
\@namedef{wv@dinov3_groups_merged_top_1@ci}{93.4 to 95.8}
\@namedef{wv@dinov3_groups_merged_top_1@lo}{93.4}
\@namedef{wv@dinov3_groups_merged_top_1@hi}{95.8}
\@namedef{wv@dinov3_minus_siglip2_top_1@v}{3.3}
\@namedef{wv@dinov3_minus_siglip2_top_1@ci}{2.1 to 4.5}
\@namedef{wv@dinov3_minus_siglip2_top_1@lo}{2.1}
\@namedef{wv@dinov3_minus_siglip2_top_1@hi}{4.5}
\@namedef{wv@dinov3_photographer_attributable@v}{1.7}
\@namedef{wv@dinov3_photographer_attributable@ci}{$-$0.3 to 3.7}
\@namedef{wv@dinov3_photographer_attributable@lo}{$-$0.3}
\@namedef{wv@dinov3_photographer_attributable@hi}{3.7}
\@namedef{wv@dinov3_photographer_raw_gap@v}{9.8}
\@namedef{wv@dinov3_photographer_raw_gap@ci}{7.0 to 12.8}
\@namedef{wv@dinov3_photographer_raw_gap@lo}{7.0}
\@namedef{wv@dinov3_photographer_raw_gap@hi}{12.8}
\@namedef{wv@dinov3_photographer_reference_cost@v}{8.1}
\@namedef{wv@dinov3_photographer_reference_cost@ci}{5.7 to 10.9}
\@namedef{wv@dinov3_photographer_reference_cost@lo}{5.7}
\@namedef{wv@dinov3_photographer_reference_cost@hi}{10.9}
\@namedef{wv@dinov3_points_per_doubling@v}{$-$0.7}
\@namedef{wv@dinov3_points_per_doubling@ci}{$-$0.8 to $-$0.5}
\@namedef{wv@dinov3_points_per_doubling@lo}{$-$0.8}
\@namedef{wv@dinov3_points_per_doubling@hi}{$-$0.5}
\@namedef{wv@dinov3_reject_cosine_auroc@v}{0.926}
\@namedef{wv@dinov3_reject_cosine_auroc@ci}{0.914 to 0.937}
\@namedef{wv@dinov3_reject_cosine_auroc@lo}{0.914}
\@namedef{wv@dinov3_reject_cosine_auroc@hi}{0.937}
\@namedef{wv@dinov3_reject_cosine_false_acceptance_90@v}{21.6}
\@namedef{wv@dinov3_reject_cosine_known_acceptance_90@v}{90.0}
\@namedef{wv@dinov3_reject_knn_auroc@v}{0.660}
\@namedef{wv@dinov3_reject_knn_auroc@ci}{0.633 to 0.689}
\@namedef{wv@dinov3_reject_knn_auroc@lo}{0.633}
\@namedef{wv@dinov3_reject_knn_auroc@hi}{0.689}
\@namedef{wv@dinov3_reject_knn_false_acceptance_90@v}{84.0}
\@namedef{wv@dinov3_reject_knn_known_acceptance_90@v}{89.9}
\@namedef{wv@dinov3_reject_knn_minus_cosine_auroc@v}{$-$0.266}
\@namedef{wv@dinov3_reject_knn_minus_cosine_auroc@ci}{$-$0.290 to $-$0.242}
\@namedef{wv@dinov3_reject_knn_minus_cosine_auroc@lo}{$-$0.290}
\@namedef{wv@dinov3_reject_knn_minus_cosine_auroc@hi}{$-$0.242}
\@namedef{wv@dinov3_reject_margin_auroc@v}{0.959}
\@namedef{wv@dinov3_reject_margin_auroc@ci}{0.949 to 0.967}
\@namedef{wv@dinov3_reject_margin_auroc@lo}{0.949}
\@namedef{wv@dinov3_reject_margin_auroc@hi}{0.967}
\@namedef{wv@dinov3_reject_margin_false_acceptance_90@v}{7.7}
\@namedef{wv@dinov3_reject_margin_known_acceptance_90@v}{89.9}
\@namedef{wv@dinov3_reject_margin_minus_cosine_auroc@v}{0.033}
\@namedef{wv@dinov3_reject_margin_minus_cosine_auroc@ci}{0.024 to 0.042}
\@namedef{wv@dinov3_reject_margin_minus_cosine_auroc@lo}{0.024}
\@namedef{wv@dinov3_reject_margin_minus_cosine_auroc@hi}{0.042}
\@namedef{wv@dinov3_soft_prior_gps10_fold_0_weight@v}{2}
\@namedef{wv@dinov3_soft_prior_gps10_fold_1_weight@v}{2}
\@namedef{wv@dinov3_soft_prior_gps10_fold_2_weight@v}{2}
\@namedef{wv@dinov3_soft_prior_gps10_fold_3_weight@v}{2}
\@namedef{wv@dinov3_soft_prior_gps10_fold_4_weight@v}{2}
\@namedef{wv@dinov3_soft_prior_gps10_gain@v}{4.3}
\@namedef{wv@dinov3_soft_prior_gps10_gain@ci}{3.3 to 5.4}
\@namedef{wv@dinov3_soft_prior_gps10_gain@lo}{3.3}
\@namedef{wv@dinov3_soft_prior_gps10_gain@hi}{5.4}
\@namedef{wv@dinov3_soft_prior_gps10_location_only_top_1@v}{90.9}
\@namedef{wv@dinov3_soft_prior_gps10_location_only_top_1@ci}{87.8 to 93.6}
\@namedef{wv@dinov3_soft_prior_gps10_location_only_top_1@lo}{87.8}
\@namedef{wv@dinov3_soft_prior_gps10_location_only_top_1@hi}{93.6}
\@namedef{wv@dinov3_soft_prior_gps10_top_1@v}{98.9}
\@namedef{wv@dinov3_soft_prior_gps10_top_1@ci}{98.1 to 99.5}
\@namedef{wv@dinov3_soft_prior_gps10_top_1@lo}{98.1}
\@namedef{wv@dinov3_soft_prior_gps10_top_1@hi}{99.5}
\@namedef{wv@dinov3_soft_prior_gps10_w0.005_top_1@v}{94.7}
\@namedef{wv@dinov3_soft_prior_gps10_w0.01_top_1@v}{94.7}
\@namedef{wv@dinov3_soft_prior_gps10_w0.02_top_1@v}{95.0}
\@namedef{wv@dinov3_soft_prior_gps10_w0.05_top_1@v}{95.5}
\@namedef{wv@dinov3_soft_prior_gps10_w0.1_top_1@v}{95.9}
\@namedef{wv@dinov3_soft_prior_gps10_w0.2_top_1@v}{97.3}
\@namedef{wv@dinov3_soft_prior_gps10_w0.5_top_1@v}{98.5}
\@namedef{wv@dinov3_soft_prior_gps10_w0_top_1@v}{94.6}
\@namedef{wv@dinov3_soft_prior_gps10_w10_top_1@v}{97.7}
\@namedef{wv@dinov3_soft_prior_gps10_w1_top_1@v}{98.8}
\@namedef{wv@dinov3_soft_prior_gps10_w20_top_1@v}{95.2}
\@namedef{wv@dinov3_soft_prior_gps10_w2_top_1@v}{98.9}
\@namedef{wv@dinov3_soft_prior_gps10_w5_top_1@v}{98.7}
\@namedef{wv@dinov3_soft_prior_gps25_fold_0_weight@v}{1}
\@namedef{wv@dinov3_soft_prior_gps25_fold_1_weight@v}{1}
\@namedef{wv@dinov3_soft_prior_gps25_fold_2_weight@v}{1}
\@namedef{wv@dinov3_soft_prior_gps25_fold_3_weight@v}{1}
\@namedef{wv@dinov3_soft_prior_gps25_fold_4_weight@v}{1}
\@namedef{wv@dinov3_soft_prior_gps25_gain@v}{3.9}
\@namedef{wv@dinov3_soft_prior_gps25_gain@ci}{3.0 to 4.9}
\@namedef{wv@dinov3_soft_prior_gps25_gain@lo}{3.0}
\@namedef{wv@dinov3_soft_prior_gps25_gain@hi}{4.9}
\@namedef{wv@dinov3_soft_prior_gps25_location_only_top_1@v}{75.1}
\@namedef{wv@dinov3_soft_prior_gps25_location_only_top_1@ci}{70.7 to 79.6}
\@namedef{wv@dinov3_soft_prior_gps25_location_only_top_1@lo}{70.7}
\@namedef{wv@dinov3_soft_prior_gps25_location_only_top_1@hi}{79.6}
\@namedef{wv@dinov3_soft_prior_gps25_top_1@v}{98.5}
\@namedef{wv@dinov3_soft_prior_gps25_top_1@ci}{97.6 to 99.2}
\@namedef{wv@dinov3_soft_prior_gps25_top_1@lo}{97.6}
\@namedef{wv@dinov3_soft_prior_gps25_top_1@hi}{99.2}
\@namedef{wv@dinov3_soft_prior_gps25_w0.005_top_1@v}{94.7}
\@namedef{wv@dinov3_soft_prior_gps25_w0.01_top_1@v}{94.7}
\@namedef{wv@dinov3_soft_prior_gps25_w0.02_top_1@v}{94.9}
\@namedef{wv@dinov3_soft_prior_gps25_w0.05_top_1@v}{95.4}
\@namedef{wv@dinov3_soft_prior_gps25_w0.1_top_1@v}{95.7}
\@namedef{wv@dinov3_soft_prior_gps25_w0.2_top_1@v}{97.3}
\@namedef{wv@dinov3_soft_prior_gps25_w0.5_top_1@v}{98.3}
\@namedef{wv@dinov3_soft_prior_gps25_w0_top_1@v}{94.6}
\@namedef{wv@dinov3_soft_prior_gps25_w10_top_1@v}{85.3}
\@namedef{wv@dinov3_soft_prior_gps25_w1_top_1@v}{98.5}
\@namedef{wv@dinov3_soft_prior_gps25_w20_top_1@v}{80.0}
\@namedef{wv@dinov3_soft_prior_gps25_w2_top_1@v}{98.2}
\@namedef{wv@dinov3_soft_prior_gps25_w5_top_1@v}{93.5}
\@namedef{wv@dinov3_soft_prior_gps50_fold_0_weight@v}{0.5}
\@namedef{wv@dinov3_soft_prior_gps50_fold_1_weight@v}{0.5}
\@namedef{wv@dinov3_soft_prior_gps50_fold_2_weight@v}{0.5}
\@namedef{wv@dinov3_soft_prior_gps50_fold_3_weight@v}{0.5}
\@namedef{wv@dinov3_soft_prior_gps50_fold_4_weight@v}{0.5}
\@namedef{wv@dinov3_soft_prior_gps50_gain@v}{3.5}
\@namedef{wv@dinov3_soft_prior_gps50_gain@ci}{2.6 to 4.4}
\@namedef{wv@dinov3_soft_prior_gps50_gain@lo}{2.6}
\@namedef{wv@dinov3_soft_prior_gps50_gain@hi}{4.4}
\@namedef{wv@dinov3_soft_prior_gps50_location_only_top_1@v}{60.2}
\@namedef{wv@dinov3_soft_prior_gps50_location_only_top_1@ci}{54.7 to 66.0}
\@namedef{wv@dinov3_soft_prior_gps50_location_only_top_1@lo}{54.7}
\@namedef{wv@dinov3_soft_prior_gps50_location_only_top_1@hi}{66.0}
\@namedef{wv@dinov3_soft_prior_gps50_top_1@v}{98.0}
\@namedef{wv@dinov3_soft_prior_gps50_top_1@ci}{97.2 to 98.8}
\@namedef{wv@dinov3_soft_prior_gps50_top_1@lo}{97.2}
\@namedef{wv@dinov3_soft_prior_gps50_top_1@hi}{98.8}
\@namedef{wv@dinov3_soft_prior_gps50_w0.005_top_1@v}{94.7}
\@namedef{wv@dinov3_soft_prior_gps50_w0.01_top_1@v}{94.7}
\@namedef{wv@dinov3_soft_prior_gps50_w0.02_top_1@v}{94.8}
\@namedef{wv@dinov3_soft_prior_gps50_w0.05_top_1@v}{95.3}
\@namedef{wv@dinov3_soft_prior_gps50_w0.1_top_1@v}{95.6}
\@namedef{wv@dinov3_soft_prior_gps50_w0.2_top_1@v}{96.7}
\@namedef{wv@dinov3_soft_prior_gps50_w0.5_top_1@v}{98.0}
\@namedef{wv@dinov3_soft_prior_gps50_w0_top_1@v}{94.6}
\@namedef{wv@dinov3_soft_prior_gps50_w10_top_1@v}{68.3}
\@namedef{wv@dinov3_soft_prior_gps50_w1_top_1@v}{97.6}
\@namedef{wv@dinov3_soft_prior_gps50_w20_top_1@v}{64.0}
\@namedef{wv@dinov3_soft_prior_gps50_w2_top_1@v}{92.9}
\@namedef{wv@dinov3_soft_prior_gps50_w5_top_1@v}{76.4}
\@namedef{wv@dinov3_soft_prior_none_top_1@v}{94.6}
\@namedef{wv@dinov3_soft_prior_none_top_1@ci}{93.3 to 95.8}
\@namedef{wv@dinov3_soft_prior_none_top_1@lo}{93.3}
\@namedef{wv@dinov3_soft_prior_none_top_1@hi}{95.8}
\@namedef{wv@dinov3_top_1@v}{94.4}
\@namedef{wv@dinov3_top_1@ci}{93.1 to 95.6}
\@namedef{wv@dinov3_top_1@lo}{93.1}
\@namedef{wv@dinov3_top_1@hi}{95.6}
\@namedef{wv@null_dinov2-large_minus_dinov2_disjoint_r_at_1@v}{2.6}
\@namedef{wv@null_dinov2-large_minus_dinov2_disjoint_r_at_1@ci}{0.5 to 4.6}
\@namedef{wv@null_dinov2-large_minus_dinov2_disjoint_r_at_1@lo}{0.5}
\@namedef{wv@null_dinov2-large_minus_dinov2_disjoint_r_at_1@hi}{4.6}
\@namedef{wv@null_dinov2-large_minus_dinov2_disjoint_r_at_10@v}{0.2}
\@namedef{wv@null_dinov2-large_minus_dinov2_disjoint_r_at_10@ci}{$-$1.1 to 1.6}
\@namedef{wv@null_dinov2-large_minus_dinov2_disjoint_r_at_10@lo}{$-$1.1}
\@namedef{wv@null_dinov2-large_minus_dinov2_disjoint_r_at_10@hi}{1.6}
\@namedef{wv@null_dinov2-registers-large_minus_dinov2_disjoint_r_at_1@v}{$-$1.0}
\@namedef{wv@null_dinov2-registers-large_minus_dinov2_disjoint_r_at_1@ci}{$-$3.3 to 1.3}
\@namedef{wv@null_dinov2-registers-large_minus_dinov2_disjoint_r_at_1@lo}{$-$3.3}
\@namedef{wv@null_dinov2-registers-large_minus_dinov2_disjoint_r_at_1@hi}{1.3}
\@namedef{wv@null_dinov2-registers-large_minus_dinov2_disjoint_r_at_10@v}{$-$1.8}
\@namedef{wv@null_dinov2-registers-large_minus_dinov2_disjoint_r_at_10@ci}{$-$3.5 to $-$0.2}
\@namedef{wv@null_dinov2-registers-large_minus_dinov2_disjoint_r_at_10@lo}{$-$3.5}
\@namedef{wv@null_dinov2-registers-large_minus_dinov2_disjoint_r_at_10@hi}{$-$0.2}
\@namedef{wv@null_dinov2-registers_minus_dinov2_disjoint_r_at_1@v}{$-$1.3}
\@namedef{wv@null_dinov2-registers_minus_dinov2_disjoint_r_at_1@ci}{$-$3.2 to 0.5}
\@namedef{wv@null_dinov2-registers_minus_dinov2_disjoint_r_at_1@lo}{$-$3.2}
\@namedef{wv@null_dinov2-registers_minus_dinov2_disjoint_r_at_1@hi}{0.5}
\@namedef{wv@null_dinov2-registers_minus_dinov2_disjoint_r_at_10@v}{$-$1.3}
\@namedef{wv@null_dinov2-registers_minus_dinov2_disjoint_r_at_10@ci}{$-$2.6 to 0.0}
\@namedef{wv@null_dinov2-registers_minus_dinov2_disjoint_r_at_10@lo}{$-$2.6}
\@namedef{wv@null_dinov2-registers_minus_dinov2_disjoint_r_at_10@hi}{0.0}
\@namedef{wv@siglip2_families_count@v}{35}
\@namedef{wv@siglip2_families_error_share@v}{14.1}
\@namedef{wv@siglip2_families_error_share@ci}{7.4 to 21.6}
\@namedef{wv@siglip2_families_error_share@lo}{7.4}
\@namedef{wv@siglip2_families_error_share@hi}{21.6}
\@namedef{wv@siglip2_families_errors@v}{149}
\@namedef{wv@siglip2_families_inside_error_rate@v}{10.1}
\@namedef{wv@siglip2_families_inside_error_rate@ci}{7.5 to 13.0}
\@namedef{wv@siglip2_families_inside_error_rate@lo}{7.5}
\@namedef{wv@siglip2_families_inside_error_rate@hi}{13.0}
\@namedef{wv@siglip2_families_outside_error_rate@v}{8.2}
\@namedef{wv@siglip2_families_outside_error_rate@ci}{6.6 to 10.0}
\@namedef{wv@siglip2_families_outside_error_rate@lo}{6.6}
\@namedef{wv@siglip2_families_outside_error_rate@hi}{10.0}
\@namedef{wv@siglip2_families_statue_share@v}{30.4}
\@namedef{wv@siglip2_families_statues@v}{93}
\@namedef{wv@siglip2_geo_minus_random_pool_10@v}{$-$1.0}
\@namedef{wv@siglip2_geo_minus_random_pool_10@ci}{$-$1.7 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_10@lo}{$-$1.7}
\@namedef{wv@siglip2_geo_minus_random_pool_10@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_100@v}{$-$0.9}
\@namedef{wv@siglip2_geo_minus_random_pool_100@ci}{$-$1.5 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_100@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_100@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_150@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_150@ci}{$-$1.4 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_150@lo}{$-$1.4}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_150@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_50@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_50@ci}{$-$1.4 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_50@lo}{$-$1.4}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_50@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_9@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_9@ci}{$-$1.5 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_9@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_100_noise_9@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_150@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_150@ci}{$-$1.3 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_150@lo}{$-$1.3}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_150@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_50@v}{$-$1.0}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_50@ci}{$-$1.7 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_50@lo}{$-$1.7}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_50@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_9@v}{$-$0.9}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_9@ci}{$-$1.7 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_9@lo}{$-$1.7}
\@namedef{wv@siglip2_geo_minus_random_pool_10_noise_9@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_15@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_15@ci}{$-$1.5 to $-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_15@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_15@hi}{$-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_150@v}{$-$0.7}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_150@ci}{$-$1.2 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_150@lo}{$-$1.2}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_150@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_50@v}{$-$0.7}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_50@ci}{$-$1.4 to $-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_50@lo}{$-$1.4}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_50@hi}{$-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_9@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_9@ci}{$-$1.5 to $-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_9@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_15_noise_9@hi}{$-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_2@v}{$-$0.6}
\@namedef{wv@siglip2_geo_minus_random_pool_2@ci}{$-$1.3 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_2@lo}{$-$1.3}
\@namedef{wv@siglip2_geo_minus_random_pool_2@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_20@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_20@ci}{$-$1.6 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_20@lo}{$-$1.6}
\@namedef{wv@siglip2_geo_minus_random_pool_20@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_200@v}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_200@ci}{$-$0.4 to 0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200@lo}{$-$0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200@hi}{0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_150@v}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_150@ci}{$-$0.4 to 0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_150@lo}{$-$0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_150@hi}{0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_50@v}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_50@ci}{$-$0.4 to 0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_50@lo}{$-$0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_50@hi}{0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_9@v}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_9@ci}{$-$0.4 to 0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_9@lo}{$-$0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_200_noise_9@hi}{0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_150@v}{$-$0.7}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_150@ci}{$-$1.3 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_150@lo}{$-$1.3}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_150@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_50@v}{$-$0.9}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_50@ci}{$-$1.5 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_50@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_50@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_9@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_9@ci}{$-$1.5 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_9@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_20_noise_9@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_294@v}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294@ci}{0.0 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294@lo}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_150@v}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_150@ci}{0.0 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_150@lo}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_150@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_50@v}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_50@ci}{0.0 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_50@lo}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_50@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_9@v}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_9@ci}{0.0 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_9@lo}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_294_noise_9@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_150@v}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_150@ci}{$-$0.6 to 0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_150@lo}{$-$0.6}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_150@hi}{0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_50@v}{$-$0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_50@ci}{$-$0.9 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_50@lo}{$-$0.9}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_50@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_9@v}{$-$0.7}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_9@ci}{$-$1.2 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_9@lo}{$-$1.2}
\@namedef{wv@siglip2_geo_minus_random_pool_2_noise_9@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_3@v}{$-$0.7}
\@namedef{wv@siglip2_geo_minus_random_pool_3@ci}{$-$1.4 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_3@lo}{$-$1.4}
\@namedef{wv@siglip2_geo_minus_random_pool_3@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_150@v}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_150@ci}{$-$0.7 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_150@lo}{$-$0.7}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_150@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_50@v}{$-$0.6}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_50@ci}{$-$1.1 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_50@lo}{$-$1.1}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_50@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_9@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_9@ci}{$-$1.5 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_9@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_3_noise_9@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_5@v}{$-$1.0}
\@namedef{wv@siglip2_geo_minus_random_pool_5@ci}{$-$1.7 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_5@lo}{$-$1.7}
\@namedef{wv@siglip2_geo_minus_random_pool_5@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_50@v}{$-$0.9}
\@namedef{wv@siglip2_geo_minus_random_pool_50@ci}{$-$1.5 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_50@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_50@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_150@v}{$-$0.9}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_150@ci}{$-$1.6 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_150@lo}{$-$1.6}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_150@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_50@v}{$-$0.9}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_50@ci}{$-$1.6 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_50@lo}{$-$1.6}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_50@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_9@v}{$-$1.0}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_9@ci}{$-$1.6 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_9@lo}{$-$1.6}
\@namedef{wv@siglip2_geo_minus_random_pool_50_noise_9@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_150@v}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_150@ci}{$-$0.6 to 0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_150@lo}{$-$0.6}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_150@hi}{0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_50@v}{$-$0.6}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_50@ci}{$-$1.3 to $-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_50@lo}{$-$1.3}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_50@hi}{$-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_9@v}{$-$0.9}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_9@ci}{$-$1.7 to $-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_9@lo}{$-$1.7}
\@namedef{wv@siglip2_geo_minus_random_pool_5_noise_9@hi}{$-$0.3}
\@namedef{wv@siglip2_geo_minus_random_pool_8@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_8@ci}{$-$1.5 to $-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_8@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_8@hi}{$-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_150@v}{$-$0.4}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_150@ci}{$-$0.8 to 0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_150@lo}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_150@hi}{0.0}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_50@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_50@ci}{$-$1.4 to $-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_50@lo}{$-$1.4}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_50@hi}{$-$0.2}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_9@v}{$-$0.8}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_9@ci}{$-$1.5 to $-$0.1}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_9@lo}{$-$1.5}
\@namedef{wv@siglip2_geo_minus_random_pool_8_noise_9@hi}{$-$0.1}
\@namedef{wv@siglip2_geo_permutation_mean_null@v}{0.0}
\@namedef{wv@siglip2_geo_permutation_mean_null@ci}{$-$0.4 to 0.4}
\@namedef{wv@siglip2_geo_permutation_mean_null@lo}{$-$0.4}
\@namedef{wv@siglip2_geo_permutation_mean_null@hi}{0.4}
\@namedef{wv@siglip2_geo_permutation_mean_observed@v}{$-$0.9}
\@namedef{wv@siglip2_geo_permutation_mean_p_value@v}{0.005}
\@namedef{wv@siglip2_geo_permutation_permutations@v}{200}
\@namedef{wv@siglip2_geo_permutation_pool_10_null_mean@v}{$-$0.1}
\@namedef{wv@siglip2_geo_permutation_pool_10_null_mean@ci}{$-$0.6 to 0.3}
\@namedef{wv@siglip2_geo_permutation_pool_10_null_mean@lo}{$-$0.6}
\@namedef{wv@siglip2_geo_permutation_pool_10_null_mean@hi}{0.3}
\@namedef{wv@siglip2_geo_permutation_pool_10_p_value@v}{0.005}
\@namedef{wv@siglip2_geo_permutation_pool_20_null_mean@v}{0.1}
\@namedef{wv@siglip2_geo_permutation_pool_20_null_mean@ci}{$-$0.4 to 0.5}
\@namedef{wv@siglip2_geo_permutation_pool_20_null_mean@lo}{$-$0.4}
\@namedef{wv@siglip2_geo_permutation_pool_20_null_mean@hi}{0.5}
\@namedef{wv@siglip2_geo_permutation_pool_20_p_value@v}{0.005}
\@namedef{wv@siglip2_geo_permutation_pool_5_null_mean@v}{0.0}
\@namedef{wv@siglip2_geo_permutation_pool_5_null_mean@ci}{$-$0.4 to 0.5}
\@namedef{wv@siglip2_geo_permutation_pool_5_null_mean@lo}{$-$0.4}
\@namedef{wv@siglip2_geo_permutation_pool_5_null_mean@hi}{0.5}
\@namedef{wv@siglip2_geo_permutation_pool_5_p_value@v}{0.005}
\@namedef{wv@siglip2_groups_changed_queries@v}{6}
\@namedef{wv@siglip2_groups_merged_gain@v}{0.4}
\@namedef{wv@siglip2_groups_merged_gain@ci}{0.0 to 0.9}
\@namedef{wv@siglip2_groups_merged_gain@lo}{0.0}
\@namedef{wv@siglip2_groups_merged_gain@hi}{0.9}
\@namedef{wv@siglip2_groups_merged_top_1@v}{91.5}
\@namedef{wv@siglip2_groups_merged_top_1@ci}{90.0 to 92.9}
\@namedef{wv@siglip2_groups_merged_top_1@lo}{90.0}
\@namedef{wv@siglip2_groups_merged_top_1@hi}{92.9}
\@namedef{wv@siglip2_photographer_attributable@v}{6.2}
\@namedef{wv@siglip2_photographer_attributable@ci}{3.9 to 8.7}
\@namedef{wv@siglip2_photographer_attributable@lo}{3.9}
\@namedef{wv@siglip2_photographer_attributable@hi}{8.7}
\@namedef{wv@siglip2_photographer_raw_gap@v}{17.2}
\@namedef{wv@siglip2_photographer_raw_gap@ci}{13.7 to 20.9}
\@namedef{wv@siglip2_photographer_raw_gap@lo}{13.7}
\@namedef{wv@siglip2_photographer_raw_gap@hi}{20.9}
\@namedef{wv@siglip2_photographer_reference_cost@v}{11.0}
\@namedef{wv@siglip2_photographer_reference_cost@ci}{8.2 to 14.2}
\@namedef{wv@siglip2_photographer_reference_cost@lo}{8.2}
\@namedef{wv@siglip2_photographer_reference_cost@hi}{14.2}
\@namedef{wv@siglip2_points_per_doubling@v}{$-$1.0}
\@namedef{wv@siglip2_points_per_doubling@ci}{$-$1.2 to $-$0.8}
\@namedef{wv@siglip2_points_per_doubling@lo}{$-$1.2}
\@namedef{wv@siglip2_points_per_doubling@hi}{$-$0.8}
\@namedef{wv@siglip2_reject_cosine_auroc@v}{0.877}
\@namedef{wv@siglip2_reject_cosine_auroc@ci}{0.861 to 0.892}
\@namedef{wv@siglip2_reject_cosine_auroc@lo}{0.861}
\@namedef{wv@siglip2_reject_cosine_auroc@hi}{0.892}
\@namedef{wv@siglip2_reject_cosine_false_acceptance_90@v}{43.8}
\@namedef{wv@siglip2_reject_cosine_known_acceptance_90@v}{89.9}
\@namedef{wv@siglip2_reject_knn_auroc@v}{0.630}
\@namedef{wv@siglip2_reject_knn_auroc@ci}{0.607 to 0.655}
\@namedef{wv@siglip2_reject_knn_auroc@lo}{0.607}
\@namedef{wv@siglip2_reject_knn_auroc@hi}{0.655}
\@namedef{wv@siglip2_reject_knn_false_acceptance_90@v}{83.1}
\@namedef{wv@siglip2_reject_knn_known_acceptance_90@v}{90.0}
\@namedef{wv@siglip2_reject_knn_minus_cosine_auroc@v}{$-$0.247}
\@namedef{wv@siglip2_reject_knn_minus_cosine_auroc@ci}{$-$0.266 to $-$0.228}
\@namedef{wv@siglip2_reject_knn_minus_cosine_auroc@lo}{$-$0.266}
\@namedef{wv@siglip2_reject_knn_minus_cosine_auroc@hi}{$-$0.228}
\@namedef{wv@siglip2_reject_margin_auroc@v}{0.916}
\@namedef{wv@siglip2_reject_margin_auroc@ci}{0.902 to 0.929}
\@namedef{wv@siglip2_reject_margin_auroc@lo}{0.902}
\@namedef{wv@siglip2_reject_margin_auroc@hi}{0.929}
\@namedef{wv@siglip2_reject_margin_false_acceptance_90@v}{27.7}
\@namedef{wv@siglip2_reject_margin_known_acceptance_90@v}{89.9}
\@namedef{wv@siglip2_reject_margin_minus_cosine_auroc@v}{0.039}
\@namedef{wv@siglip2_reject_margin_minus_cosine_auroc@ci}{0.027 to 0.051}
\@namedef{wv@siglip2_reject_margin_minus_cosine_auroc@lo}{0.027}
\@namedef{wv@siglip2_reject_margin_minus_cosine_auroc@hi}{0.051}
\@namedef{wv@siglip2_soft_prior_gps10_fold_0_weight@v}{1}
\@namedef{wv@siglip2_soft_prior_gps10_fold_1_weight@v}{1}
\@namedef{wv@siglip2_soft_prior_gps10_fold_2_weight@v}{1}
\@namedef{wv@siglip2_soft_prior_gps10_fold_3_weight@v}{1}
\@namedef{wv@siglip2_soft_prior_gps10_fold_4_weight@v}{1}
\@namedef{wv@siglip2_soft_prior_gps10_gain@v}{7.6}
\@namedef{wv@siglip2_soft_prior_gps10_gain@ci}{6.3 to 9.0}
\@namedef{wv@siglip2_soft_prior_gps10_gain@lo}{6.3}
\@namedef{wv@siglip2_soft_prior_gps10_gain@hi}{9.0}
\@namedef{wv@siglip2_soft_prior_gps10_location_only_top_1@v}{90.8}
\@namedef{wv@siglip2_soft_prior_gps10_location_only_top_1@ci}{87.8 to 93.4}
\@namedef{wv@siglip2_soft_prior_gps10_location_only_top_1@lo}{87.8}
\@namedef{wv@siglip2_soft_prior_gps10_location_only_top_1@hi}{93.4}
\@namedef{wv@siglip2_soft_prior_gps10_top_1@v}{99.0}
\@namedef{wv@siglip2_soft_prior_gps10_top_1@ci}{98.4 to 99.6}
\@namedef{wv@siglip2_soft_prior_gps10_top_1@lo}{98.4}
\@namedef{wv@siglip2_soft_prior_gps10_top_1@hi}{99.6}
\@namedef{wv@siglip2_soft_prior_gps10_w0.005_top_1@v}{91.8}
\@namedef{wv@siglip2_soft_prior_gps10_w0.01_top_1@v}{92.3}
\@namedef{wv@siglip2_soft_prior_gps10_w0.02_top_1@v}{93.5}
\@namedef{wv@siglip2_soft_prior_gps10_w0.05_top_1@v}{95.4}
\@namedef{wv@siglip2_soft_prior_gps10_w0.1_top_1@v}{96.6}
\@namedef{wv@siglip2_soft_prior_gps10_w0.2_top_1@v}{98.0}
\@namedef{wv@siglip2_soft_prior_gps10_w0.5_top_1@v}{98.8}
\@namedef{wv@siglip2_soft_prior_gps10_w0_top_1@v}{91.4}
\@namedef{wv@siglip2_soft_prior_gps10_w10_top_1@v}{94.4}
\@namedef{wv@siglip2_soft_prior_gps10_w1_top_1@v}{99.0}
\@namedef{wv@siglip2_soft_prior_gps10_w20_top_1@v}{93.0}
\@namedef{wv@siglip2_soft_prior_gps10_w2_top_1@v}{98.8}
\@namedef{wv@siglip2_soft_prior_gps10_w5_top_1@v}{97.1}
\@namedef{wv@siglip2_soft_prior_gps25_fold_0_weight@v}{0.5}
\@namedef{wv@siglip2_soft_prior_gps25_fold_1_weight@v}{0.5}
\@namedef{wv@siglip2_soft_prior_gps25_fold_2_weight@v}{0.5}
\@namedef{wv@siglip2_soft_prior_gps25_fold_3_weight@v}{0.5}
\@namedef{wv@siglip2_soft_prior_gps25_fold_4_weight@v}{0.5}
\@namedef{wv@siglip2_soft_prior_gps25_gain@v}{6.9}
\@namedef{wv@siglip2_soft_prior_gps25_gain@ci}{5.6 to 8.2}
\@namedef{wv@siglip2_soft_prior_gps25_gain@lo}{5.6}
\@namedef{wv@siglip2_soft_prior_gps25_gain@hi}{8.2}
\@namedef{wv@siglip2_soft_prior_gps25_location_only_top_1@v}{75.0}
\@namedef{wv@siglip2_soft_prior_gps25_location_only_top_1@ci}{70.4 to 79.4}
\@namedef{wv@siglip2_soft_prior_gps25_location_only_top_1@lo}{70.4}
\@namedef{wv@siglip2_soft_prior_gps25_location_only_top_1@hi}{79.4}
\@namedef{wv@siglip2_soft_prior_gps25_top_1@v}{98.3}
\@namedef{wv@siglip2_soft_prior_gps25_top_1@ci}{97.5 to 98.9}
\@namedef{wv@siglip2_soft_prior_gps25_top_1@lo}{97.5}
\@namedef{wv@siglip2_soft_prior_gps25_top_1@hi}{98.9}
\@namedef{wv@siglip2_soft_prior_gps25_w0.005_top_1@v}{91.8}
\@namedef{wv@siglip2_soft_prior_gps25_w0.01_top_1@v}{92.2}
\@namedef{wv@siglip2_soft_prior_gps25_w0.02_top_1@v}{93.4}
\@namedef{wv@siglip2_soft_prior_gps25_w0.05_top_1@v}{95.3}
\@namedef{wv@siglip2_soft_prior_gps25_w0.1_top_1@v}{96.3}
\@namedef{wv@siglip2_soft_prior_gps25_w0.2_top_1@v}{97.6}
\@namedef{wv@siglip2_soft_prior_gps25_w0.5_top_1@v}{98.3}
\@namedef{wv@siglip2_soft_prior_gps25_w0_top_1@v}{91.4}
\@namedef{wv@siglip2_soft_prior_gps25_w10_top_1@v}{78.9}
\@namedef{wv@siglip2_soft_prior_gps25_w1_top_1@v}{97.5}
\@namedef{wv@siglip2_soft_prior_gps25_w20_top_1@v}{77.1}
\@namedef{wv@siglip2_soft_prior_gps25_w2_top_1@v}{92.9}
\@namedef{wv@siglip2_soft_prior_gps25_w5_top_1@v}{82.9}
\@namedef{wv@siglip2_soft_prior_gps50_fold_0_weight@v}{0.2}
\@namedef{wv@siglip2_soft_prior_gps50_fold_1_weight@v}{0.2}
\@namedef{wv@siglip2_soft_prior_gps50_fold_2_weight@v}{0.2}
\@namedef{wv@siglip2_soft_prior_gps50_fold_3_weight@v}{0.2}
\@namedef{wv@siglip2_soft_prior_gps50_fold_4_weight@v}{0.2}
\@namedef{wv@siglip2_soft_prior_gps50_gain@v}{5.5}
\@namedef{wv@siglip2_soft_prior_gps50_gain@ci}{4.3 to 6.8}
\@namedef{wv@siglip2_soft_prior_gps50_gain@lo}{4.3}
\@namedef{wv@siglip2_soft_prior_gps50_gain@hi}{6.8}
\@namedef{wv@siglip2_soft_prior_gps50_location_only_top_1@v}{60.1}
\@namedef{wv@siglip2_soft_prior_gps50_location_only_top_1@ci}{54.7 to 65.8}
\@namedef{wv@siglip2_soft_prior_gps50_location_only_top_1@lo}{54.7}
\@namedef{wv@siglip2_soft_prior_gps50_location_only_top_1@hi}{65.8}
\@namedef{wv@siglip2_soft_prior_gps50_top_1@v}{96.9}
\@namedef{wv@siglip2_soft_prior_gps50_top_1@ci}{96.0 to 97.7}
\@namedef{wv@siglip2_soft_prior_gps50_top_1@lo}{96.0}
\@namedef{wv@siglip2_soft_prior_gps50_top_1@hi}{97.7}
\@namedef{wv@siglip2_soft_prior_gps50_w0.005_top_1@v}{91.8}
\@namedef{wv@siglip2_soft_prior_gps50_w0.01_top_1@v}{92.1}
\@namedef{wv@siglip2_soft_prior_gps50_w0.02_top_1@v}{93.1}
\@namedef{wv@siglip2_soft_prior_gps50_w0.05_top_1@v}{94.9}
\@namedef{wv@siglip2_soft_prior_gps50_w0.1_top_1@v}{95.9}
\@namedef{wv@siglip2_soft_prior_gps50_w0.2_top_1@v}{96.9}
\@namedef{wv@siglip2_soft_prior_gps50_w0.5_top_1@v}{95.8}
\@namedef{wv@siglip2_soft_prior_gps50_w0_top_1@v}{91.4}
\@namedef{wv@siglip2_soft_prior_gps50_w10_top_1@v}{63.1}
\@namedef{wv@siglip2_soft_prior_gps50_w1_top_1@v}{87.8}
\@namedef{wv@siglip2_soft_prior_gps50_w20_top_1@v}{61.7}
\@namedef{wv@siglip2_soft_prior_gps50_w2_top_1@v}{75.4}
\@namedef{wv@siglip2_soft_prior_gps50_w5_top_1@v}{66.1}
\@namedef{wv@siglip2_soft_prior_none_top_1@v}{91.4}
\@namedef{wv@siglip2_soft_prior_none_top_1@ci}{89.9 to 92.9}
\@namedef{wv@siglip2_soft_prior_none_top_1@lo}{89.9}
\@namedef{wv@siglip2_soft_prior_none_top_1@hi}{92.9}
\@namedef{wv@siglip2_top_1@v}{91.2}
\@namedef{wv@siglip2_top_1@ci}{89.6 to 92.6}
\@namedef{wv@siglip2_top_1@lo}{89.6}
\@namedef{wv@siglip2_top_1@hi}{92.6}
\makeatother


==> generated/sens-numbers.tex <==
\makeatletter
\@namedef{wv@sens_cap_disk_lightglue_max_gain@v}{2.5}
\@namedef{wv@sens_cap_disk_lightglue_min_gain@v}{1.4}
\@namedef{wv@sens_cap_loftr_max_gain@v}{4.1}
\@namedef{wv@sens_cap_loftr_min_gain@v}{0.2}
\@namedef{wv@sens_cap_sift_max_gain@v}{0.6}
\@namedef{wv@sens_cap_sift_min_gain@v}{$-$0.2}
\@namedef{wv@sens_prior_gps100_max_top_1@v}{97.5}
\@namedef{wv@sens_prior_gps100_min_top_1@v}{93.6}
\@namedef{wv@sens_prior_gps10_max_top_1@v}{99.2}
\@namedef{wv@sens_prior_gps10_min_top_1@v}{98.4}
\@namedef{wv@sens_prior_gps25_max_top_1@v}{98.8}
\@namedef{wv@sens_prior_gps25_min_top_1@v}{97.7}
\@namedef{wv@sens_prior_gps50_max_top_1@v}{98.3}
\@namedef{wv@sens_prior_gps50_min_top_1@v}{95.3}
\@namedef{wv@sens_prior_runs_count@v}{10}
\makeatother

